MotherNets: Rapid Deep Ensemble Learning

Ensembles of deep neural networks significantly improve generalization accuracy. However, training neural network ensembles requires a large amount of computational resources and time. State-of-the-art approaches either train all networks from scratch leading to prohibitive training cost that allows only very small ensemble sizes in practice, or generate ensembles by training a monolithic architecture, which results in lower model diversity and decreased prediction accuracy. We propose MotherNets to enable higher accuracy and practical training cost for large and diverse neural network ensembles: A MotherNet captures the structural similarity across some or all members of a deep neural network ensemble which allows us to share data movement and computation costs across these networks. We first train a single or a small set of MotherNets and, subsequently, we generate the target ensemble networks by transferring the function from the trained MotherNet(s). Then, we continue to train these ensemble networks, which now converge drastically faster compared to training from scratch. MotherNets handle ensembles with diverse architectures by clustering ensemble networks of similar architecture and training a separate MotherNet for every cluster. MotherNets also use clustering to control the accuracy vs. training cost tradeoff. We show that compared to state-of-the-art approaches such as Snapshot Ensembles, Knowledge Distillation, and TreeNets, MotherNets provide a new Pareto frontier for the accuracy-training cost tradeoff. Crucially, training cost and accuracy improvements continue to scale as we increase the ensemble size (2 to 3 percent reduced absolute test error rate and up to 35 percent faster training compared to Snapshot Ensembles). We verify these benefits over numerous neural network architectures and large data sets.

==> files/FPT.tex <==
\section{Function-Preserving Transformation}

\begin{figure*}[h!]
	\includegraphics[width=\linewidth]{images/schematic/FPT}
	\caption{\label{fig:FPT} Function-preserving transformations used 
	to tranfer knowledge between the MotherNet and the ensembles.}
\end{figure*}

We provide an overview of function-preserving transformations 
that we use to transfer knowledge between a trained MotherNet 
and ensemble networks. 

\boldPara{Function-preserving transformations.} 
% Overview:
Function-preserving transformations allow us to grow the size of 
a neural network i.e., increase its model capacity, while ensuring 
that the function it represents is preserved 
\cite{Chen2015,Wei2016,Wei2017}. 
% Formal
Formally, let $N$ be a neural network with parameters $\boldtheta$, 
such that it can be represented by a function $\boldy = 
f(\boldx,\boldtheta)$, where $\boldx$ is the input to the network and 
$\boldy$ is the output from the network. 
%
Function-preserving transformations allow us to construct another 
network $N'$ with parameters $\boldtheta'$ such that its function 
$g(\boldx,\boldtheta')$ is the same as that of $N$. In particular, 
the following holds: 

\begin{equation}
	\forall \boldx, g(\boldx,\boldtheta') = f(\boldx,\boldtheta) 
	\label{eq:FPT}		
\end{equation}

% Two approaches:
There are two approaches to achieve this: Net2Net and Network 
Morphism. 
% Net2Net and NetMorph
Net2Net increases the capacity of the given network by adding 
identity layers or by replicating existing weights \cite{Chen2015}. 
Network Morphism, on the other hand, derives sufficient and 
necessary conditions that when satisfied will extend the network 
while preserving its function and, it provides explicit algorithms 
to solve for those conditions \cite{Wei2016,Wei2017}. 
%
Function-preserving transformations readily exist for all 
feed-forward neural network architectures including 
state-of-the-art architectures such as ResNets, DenseNets, 
and MobileNets \cite{Cai2017}.  


We use three different classes of function-preserving 
transformations that we describe in detail below: 

\boldPara{Deepen Networks.} 
%
This transformation allows us to increase the depth of the network 
by adding a new layer as shown in Figure \ref{fig:FPT}a.
%
Specifically, this transformation replaces a layer in the network 
$\boldB_{l+1} = \boldG \cdot \boldB_{l-1}$ with two layers 
$\boldB_{l+1} = \boldF_{l+1} \cdot \boldF_{l} \cdot \boldB_{l-1}$. 
%
For this transformation to be function-preserving, the following 
should hold: 

\begin{equation}
\boldG = \boldF_{l+1} \cdot \boldF_{l}	
	\label{eq:net2deepernet}
\end{equation}


In Net2Net, the above condition is achieved by setting $\boldF_l$ 
to $\boldG$ and $\boldF_{l+1}$ to the identity matrix \cite{Chen2015}. 
%
For ResNets, we initialize $\boldF_l$ to $\boldG$ and $\boldF_{l+1}$ 
to a zero matrix. This is because of skip-connections that concatenate 
the output of the previous layer with the next layer \cite{He2016}. 
%
Network Morphism, on the other hand, uses deconvolution-based 
algorithms to solve Equation \ref{eq:net2deepernet} with the added 
constraints that: 
(i) both $\boldF_l$ and $\boldF_{l+1}$ contain as many non-zero elements 
as possible and (ii) the parameters are in consistent scale 
\cite{Wei2016}. 
%

\boldPara{Widen Networks.} 
%
This transformation allows us to increase the width of a layer in the 
network by adding new units or, in the case of convolutional layers, 
adding new convolutional channels or filters. 
%
Suppose we have two fully-connected layers $i$ and $i+1$ with 
weight matrices $\boldW^{(i)} \in \mathbb{R}^{m \times n}$ and 
$\boldW^{(i+1)} \in \mathbb{R}^{n \times p}$, to widen layer $i$ 
(i.e., increase its output from $n$ to $q$, where $q > n$), we 
introduce two new weight matrices 
$\boldU^{(i)} \in \mathbb{R}^{m \times q}$ and $\boldU^{(i+1)} \in 
\mathbb{R}^{n \times p}$ and construct them as follows: The 
first $n$ columns of $\boldW^{(i)}$ are copied directly into $\boldU^{(i)}$, 
the rest of the $q - n$ columns are initialized by randomly 
choosing one of the columns from $\boldW^{(i)}$ with replacement. The 
weights in $\boldU^{(i+1)}$ that correspond to replicated columns 
$\boldU^{(i)}$ are then adjusted by dividing those weights by the 
replication factor. 
%
For instance, in Figure \ref{fig:FPT}b, the unit labelled `a' is 
replicated. To account for this replication, the corresponding 
weight in the next layer is divided by the replication factor, 
in this case $2$. 
%
In the case of convolutional neural networks, where several units 
share the same weight, the replication happens at the level of 
convolutional channels instead of individual units \cite{Chen2015}. 
%

\boldPara{Enlarge Convolutional Filters.} 
This transformation allows us to increase the size of the 
filters or convolutional channels in a convolutional layer 
as shown in Figure \ref{fig:FPT}c.
% Setup 
Suppose we have a convolutional layer $i$ and its input is 
represented by a three-dimensional matrix 
$\boldW_i \in \mathbb{R}^{w \times h \times d}$. 
Associated with this input layer is a set 
$F = \{\boldF_0,\boldF_1, \dots \boldF_{K-1}\}$ of three-dimensional filters, 
where $\boldF_k \in \mathbb{R}^{f \times f \times d}$. When this 
set of filters is applied to the input matrix, with a stride 
of length one, we get an output layer $i+1$ represented by 
a three-dimensional matrix $\boldW_{i+1} \in \mathbb{R}^{(w-f+1) 
\times (h-f+1) \times K}$. To enlarge the filters, we replace $F$ with 
a set of enlarged filters $F'$, such that $\boldF'_k \in \mathbb{R}^{(f+x) 
\times (f+x) \times d}$. 
%
To achieve this, both the filter and the input layer volume are 
padded with zeros of width $x/2$ on each side. This preserves 
both the dimensions as well as the values in the output layer. 

\boldPara{Adding random noise.} 
\rev{Function-preserving transformations introduce additional 
parameters to the network that can be further trained. Before 
further training these parameters, we add small random noise to 
the newly introduced weights. This random noise is helpful as 
(i) it creates diversity; and (ii) overcomes the vanishing 
gradient problem that may occur due to introduction of 
identity matrices and zeroed out weights. This results in 
faster convergence of the network to a different minima.} 

%
%The upper left volume of $\boldF'_k$ is the 
%same as $\boldF_k$, whereas the rest of the volume is initialized to 
%zeros. 
%%
%Now that the filter is enlarged, convolving this filter will result 
%in a smaller output layer of volume $(w-f-x+1) \times (h-f-x+1) 
%\times K$. To compensate for this, the input matrix 
%$\boldW_i$ is also enlarged to $\boldU_i \in \mathbb{R}^{(w+x) \times (h+x) 
%\times d}$ and constructed in a similar fashion, where the upper 
%left volume of $\boldU_i$ is the same as $\boldW_i$ and the rest 
%of it is initialized to zeros. 
%



% Intro + overview
%Net2DeeperNet and Net2WiderNet do not allow us to grow the filter 
%size of a convolutional layer. To complement them, we introduce 
%a novel function-preserving transformation EnlargeFilter, which 
%allows us to grow the filter size of convolutional layers. 
%% Net2ResNet
%\boldPara{Net2ResNet.} 
%% A brief intro to ResNets 
%Residual networks use skip-connections to connect input from 
%one layer of the network to the output from a subsequent layer 
%\cite{He2016}. In particular, assume two layers with input 
%vectors $\boldx$ and output vector $\boldy$. Introducing a 
%skip connection between these two layers results in the following 
%transformation: 
%
%\begin{equation}
%\boldy = g(F(\boldx,\{\boldW_i\})) \longrightarrow 
%g(F(\boldx,\{\boldW_i\}) + \boldW_s \boldx)	
%\label{eq:resnet}
%\end{equation}
%
%Here $W_s$ is the scaling matrix that allows the dimensions 
%of $\boldx$ to match with the dimensions of $F(\boldx,\{\boldW_i\})$ 
%and $g$ is the non-linearity (e.g., ReLU). Though, the above 
%notations are in terms of fully-connected layers, they are applicable 
%to convolutional layers -- the element-wise addition is performed 
%filter-by-filter. Net2ResNet allows us to add skip connections 
%(i.e., perform the transformation in Equation \ref{eq:resnet}) 
%in a function-preserving manner. To achieve this, we introduce an 
%adjustment matrix $\boldU$ and perform element-wise product of 
%this matrix with $F + \boldW_s \boldx$. This matrix has the same 
%dimension as $F + \boldW_s \boldx$ and is constructed as follows: 
%
%$$
%\boldU_i = \frac{F_i}{\{F + \boldW_s x\}_i}
%$$ 
%
%The overall transformation now becomes: 
%
%\begin{equation}
%\boldy = g(F(\boldx,\{\boldW_i\})) \longrightarrow g(F(\boldx,\{\boldW_i\}) + \boldW_s \boldx) \longrightarrow g((F(\boldx,\{\boldW_i\}) + \boldW_s \boldx) 
%\otimes U)
%\label{eq:resnet}
%\end{equation}




%% Detailed explanation 

%\todo{In practice, how does the newly added parts of the filter change?}

%
%
%is applied such that 
%$\boldF_i = f \times f \times h$ 
%are applied to generate the output matrix $\boldW_{i+1} \in 
%\mathbb{R}^{(w-f+1) \times (h-f+1) \times k}$. 
%
%
%
%with spatial dimension 
%$w_i \times h_i$ and depth $d_i$. To generate layer $i+1$, output from 
%this layer is passed on to the next layer that has $k_i$ square filters 
%of spatial dimension $f_i \times f_i$ and depth $d_i$. If the size of 
%the stride is set to $1$, layer $i+1$ has spatial dimension $(w_i - f_i)+1 
%\times (h_i - f_i)+1$ and depth $k_i$. 
%%
%Net2WiderNet expands the filter size from $f_i \times f_i$ to 
%$f'_i \times f'_i$, where $f' = f + x$. For every depth of the 
%filter, the first $f_i \times f_i$ are the same 


% 


%\section{Function-preserving transformations} 
%
%We provide a detailed overview of function-preserving transformations. 
%They allow us to grow the size of a neural network, while ensuring 
%that the function it represents is preserved. 
%%
%Function-preserving transformations enable the ensemble networks to 
%\textit{inherit} the learnt function from the MotherNet. 
%%
%We use three classes of function-preserving transformations 
%as shown in Figure \ref{fig:FPT} and they allow us to increase the 
%depth of the network (Figure \ref{fig:FPT}a), widen the network 
%layers (Figure \ref{fig:FPT}b), and grow the size of convolutional 
%filters (Figure \ref{fig:FPT}c). 
%% 
%There are two distinct approaches to achieve these transformations: 
%Net2Net and Network Morphism. 
%%
%Net2Net increases the capacity of the given network by adding identity 
%layers or by replicating existing weights \cite{Chen2015}. 
%%
%Network Morphism, on the other hand, derives sufficient and necessary 
%conditions that when satisfied will extend the network while preserving 
%its function and provides algorithms to solve for those conditions 
%\cite{Wei2016,Wei2017}. 
%%
%In MotherNet, we adopt the second approach 
%\footnote{There is ongoing research on function-preserving 
%transformations. Novel and better approaches introduced in 
%the future can also be applied within the context of 
%MotherNets.} 
%i.e., Network Morphism, as 
%it has been shown to serve as a better starting point for further 
%training of the expanded network as compared to Net2Net \cite{Wei2016,Wei2017}. 
%These 
%transformations are readily applicable to a wide range of feed-forward 
%neural networks including VGGNets, ResNets, and 
%DenseNets \cite{Chen2015,Wei2016,Wei2017}.

==> files/background.tex <==
\section{Background}
\label{sec:background}

\boldPara{Function-preserving transformations.}
% Introduction 
We provide a brief overview of function-preserving 
transformations, which allow us to expand the size of 
any feed-forward neural network while ensuring that 
its function is preserved. 
%
Function-preserving transformations are widely used 
in various techniques that improve network architecture 
search as well as enable lifelong learning, and transfer 
learning \cite{Chen2015,Fernando2017,Li2017,Wei2016,Wei2017}
%
We use three classes of function-preserving transformations:
 
%as shown in Figure \ref{fig:FPT} and they allow us to increase the 
%depth of the network (Figure \ref{fig:FPT}a), widen the network 
%layers (Figure \ref{fig:FPT}b), and grow the size of convolutional 
%filters (Figure \ref{fig:FPT}c). 
%%
%Here, we provide an overview of these transformations. 
%They are explained in detail in \rev{Appendix A}. 

\boldPara{Deeper networks.}
% How?
To increase the depth of a network, a new layer with identity 
weight matrix (i.e., all weights set to $1$) is added to the 
network. 
% Why?
This new layer has the effect of multiplying the outputs of 
neurons from the previous layer with $1$. In this way, it transfers 
those weights unchanged to the layer after it.  
% e.g.,
Figure \ref{fig:FPT}a shows an example where a new layer with 
identity weight matrix $I$ is added. 
The output $O$ (shown at the bottom) of the original and 
the transformed network is the same.

\boldPara{Wider networks.}
% How?
To widen a layer in a network, a subset of the layer's neurons are 
replicated and the weights associated with the outputs of the 
replicated neurons (in the next layer) are divided by their 
replication factor. This normalization ensures that the 
replicated neurons do not alter the output of the layer. 
% e.g., 
For example, in Figure \ref{fig:FPT}b, neuron $x_1$ is 
replicated in the transformed network. To adjust for this, 
the weight associated with the replicated neuron $w_1$ is 
divided by the replication factor of $2$. The output $O$ 
remains unchanged. 


\boldPara{Larger convolutional filters.} For convolutional 
neural networks, to increase the size of convolutional filters 
both the input layer and the filter is padded with zeros on 
each side. 
% 
This transformation ensures that the output dimension and 
values remain the same as the convolutional operator (which 
is a strided matrix dot product) is not affected by zero padding. 
% e.g., 
Figure \ref{fig:FPT}c shows an example, where the input layer 
$A$ and the filter $F$ are both padded with one layer of zeros. 
The output of the convolution remains unchanged. 






% 
%There are two distinct approaches to achieve these transformations: 
%Net2Net and Network Morphism. 
%%
%Net2Net increases the capacity of the given network by adding identity 
%layers or by replicating existing weights \cite{Chen2015}. 
%%
%Network Morphism, on the other hand, derives sufficient and necessary 
%conditions that when satisfied will extend the network while preserving 
%its function and provides algorithms to solve for those conditions 
%\cite{Wei2016,Wei2017}. 
%%
%In MotherNet, we adopt the second approach 
%%\footnote{There is ongoing research on function-preserving 
%%transformations. Novel and better approaches introduced in 
%%the future can also be applied within the context of 
%%MotherNets.} 
%i.e., Network Morphism, as 
%it has been shown to serve as a better starting point for further 
%training of the expanded network as compared to Net2Net \cite{Wei2016,Wei2017}. 
%These 
%transformations are readily applicable to a wide range of feed-forward 
%neural networks including VGGNets, ResNets, FractalNets, 
%and DenseNets \cite{Chen2015,Wei2016,Wei2017}. 
%\rev{Appendix A provides a detailed discussion on function-preserving 
%transformations.}
%

==> files/bgd.tex <==
\section{Background}

We provide an overview of function-preserving transformations that 
we use to transfer knowledge between the MotherNet and the ensemble 
networks. 

\boldPara{Function-preserving transformations.} 
% Overview
Given a neural network, function-preserving transformations can 
be applied to create another neural network with more model capacity 
(parameters) than the teacher neural network while preserving its 
function \cite{Chen2015,Wei2016,Wei2017}. 
% Net2Net 
We provide an overview of two approaches to achieve this: 
Net2Net and Network Morphism. 
%
Net2Net increases the capacity of the given network by adding 
identity layers or by replicating existing weights \cite{Chen2015}. 
Network Morphism, on the other hand, derives sufficient and necessary 
conditions that when satisfied will extend the network while preserving 
its function and, it provides algorithms to solve for those conditions 
\cite{Wei2016,Wei2017}. 
%

%% Formal
%Formally, let $N$ be a neural network with parameters $\boldtheta$, 
%such that it can be represented by a function $\boldy = 
%f(\boldx,\boldtheta)$, where $\boldx$ is the input to the network and 
%$\boldy$ is the output from the network. 
%%
%Function-preserving transformations allow us to construct another 
%network $N'$ with parameters $\boldtheta'$ such that its function 
%$g(\boldx,\boldtheta')$ is the same as that of $N$. In particular, 
%the following holds: 
%
%\begin{equation}
%	\forall \boldx, g(\boldx,\boldtheta') = f(\boldx,\boldtheta) 
%	\label{eq:FPT}		
%\end{equation}

\boldPara{Deeper Networks.} 
%
This transformation allows us to increase the depth of the network 
by adding a new layer as shown in Figure \ref{fig:FPT}a.
%
Specifically, this transformation replaces a layer in the network 
$\boldB_{l+1} = \boldG \cdot \boldB_{l-1}$ with two layers 
$\boldB_{l+1} = \boldF_{l+1} \cdot \boldF_{l} \cdot \boldB_{l-1}$. 
%
For this transformation to be function-preserving, the following 
should hold: 

\begin{equation}
\boldG = \boldF_{l+1} \cdot \boldF_{l}	
	\label{eq:net2deepernet}
\end{equation}


In Net2Net, the above condition is achieved by setting $\boldF_l$ 
to $\boldG$ and $\boldF_{l+1}$ to the identity matrix \cite{Chen2015}. 
Whereas Network Morphism introduces deconvolution-based algorithms to 
solve Equation \ref{eq:net2deepernet} with the added constraints that 
(1) both $\boldF_l$ and $\boldF_{l+1}$ contain as many non-zero elements 
as possible (2) the parameters are in consistent scale 
\cite{Wei2016}. 
%
%
%\rev{Note that for ResNets, we initialize $\boldF_l$ to $\boldG$ 
%and $\boldF_{l+1}$ to a zero matrix. This is because of skip-connections 
%that concatenate the output of the previous layer with the next 
%layer \cite{He2016}.} 

\todo{Add ResNets and DenseNets ideas here.}



\boldPara{Wider Networks.} 
%
This transformation allows us to increase the width of a layer in the 
network by adding new units or, in the case of convolutional layers, 
adding new convolutional channels or filters. 
%
Suppose we have two fully-connected layers $i$ and $i+1$ with 
weight matrices $\boldW^{(i)} \in \mathbb{R}^{m \times n}$ and 
$\boldW^{(i+1)} \in \mathbb{R}^{n \times p}$, to widen layer $i$ 
(i.e., increase its output from $n$ to $q$, where $q > n$), we 
introduce two new weight matrices 
$\boldU^{(i)} \in \mathbb{R}^{m \times q}$ and $\boldU^{(i+1)} \in 
\mathbb{R}^{n \times p}$ and construct them as follows: The 
first $n$ columns of $\boldW^{(i)}$ are copied directly into $\boldU^{(i)}$, 
the rest of the $q - n$ columns are initialized by randomly 
choosing one of the columns from $\boldW^{(i)}$ with replacement. The 
weights in $\boldU^{(i+1)}$ that correspond to replicated columns 
$\boldU^{(i)}$ are then adjusted by dividing those weights by the 
replication factor. 
%
For instance, in Figure \ref{fig:FPT}b, the unit labelled `a' is 
replicated. To account for this replication, the corresponding 
weight in the next layer is divided by the replication factor, 
in this case $2$. 
%
In the case of CNNs, where several units share the same weight, 
the replication happens at the level of channels instead of 
individual units \cite{Chen2015}. 
%

\todo{Consider mentioning network morphism's approach here.}

\boldPara{Larger Convolutional Filters.} 
This transformation allows us to increase the size of the 
filters or convolutional channels in a convolutional layer 
as shown in Figure \ref{fig:FPT}c.
% Setup 
Suppose we have a convolutional layer $i$ and its input is 
represented by a three-dimensional matrix 
$\boldW_i \in \mathbb{R}^{w \times h \times d}$. 
Associated with this input layer is a set 
$F = \{\boldF_0,\boldF_1, \dots \boldF_{K-1}\}$ of three-dimensional filters, 
where $\boldF_k \in \mathbb{R}^{f \times f \times d}$. When this 
set of filters is applied to the input matrix, with a stride 
of length one, we get an output layer $i+1$ represented by 
a three-dimensional matrix $\boldW_{i+1} \in \mathbb{R}^{(w-f+1) 
\times (h-f+1) \times K}$. To enlarge the filters, we replace $F$ with 
a set of enlarged filters $F'$, such that $\boldF'_k \in \mathbb{R}^{(f+x) 
\times (f+x) \times d}$. 
%
To achieve this, both the filter and the input layer volume are 
padded with zeros of width $x/2$ on each side. This preserves 
both the dimensions as well as the values in the output layer. 

\todo{Consider mentioning how we add noise etc. }

%
%The upper left volume of $\boldF'_k$ is the 
%same as $\boldF_k$, whereas the rest of the volume is initialized to 
%zeros. 
%%
%Now that the filter is enlarged, convolving this filter will result 
%in a smaller output layer of volume $(w-f-x+1) \times (h-f-x+1) 
%\times K$. To compensate for this, the input matrix 
%$\boldW_i$ is also enlarged to $\boldU_i \in \mathbb{R}^{(w+x) \times (h+x) 
%\times d}$ and constructed in a similar fashion, where the upper 
%left volume of $\boldU_i$ is the same as $\boldW_i$ and the rest 
%of it is initialized to zeros. 
%



% Intro + overview
%Net2DeeperNet and Net2WiderNet do not allow us to grow the filter 
%size of a convolutional layer. To complement them, we introduce 
%a novel function-preserving transformation EnlargeFilter, which 
%allows us to grow the filter size of convolutional layers. 
%% Net2ResNet
%\boldPara{Net2ResNet.} 
%% A brief intro to ResNets 
%Residual networks use skip-connections to connect input from 
%one layer of the network to the output from a subsequent layer 
%\cite{He2016}. In particular, assume two layers with input 
%vectors $\boldx$ and output vector $\boldy$. Introducing a 
%skip connection between these two layers results in the following 
%transformation: 
%
%\begin{equation}
%\boldy = g(F(\boldx,\{\boldW_i\})) \longrightarrow 
%g(F(\boldx,\{\boldW_i\}) + \boldW_s \boldx)	
%\label{eq:resnet}
%\end{equation}
%
%Here $W_s$ is the scaling matrix that allows the dimensions 
%of $\boldx$ to match with the dimensions of $F(\boldx,\{\boldW_i\})$ 
%and $g$ is the non-linearity (e.g., ReLU). Though, the above 
%notations are in terms of fully-connected layers, they are applicable 
%to convolutional layers -- the element-wise addition is performed 
%filter-by-filter. Net2ResNet allows us to add skip connections 
%(i.e., perform the transformation in Equation \ref{eq:resnet}) 
%in a function-preserving manner. To achieve this, we introduce an 
%adjustment matrix $\boldU$ and perform element-wise product of 
%this matrix with $F + \boldW_s \boldx$. This matrix has the same 
%dimension as $F + \boldW_s \boldx$ and is constructed as follows: 
%
%$$
%\boldU_i = \frac{F_i}{\{F + \boldW_s x\}_i}
%$$ 
%
%The overall transformation now becomes: 
%
%\begin{equation}
%\boldy = g(F(\boldx,\{\boldW_i\})) \longrightarrow g(F(\boldx,\{\boldW_i\}) + \boldW_s \boldx) \longrightarrow g((F(\boldx,\{\boldW_i\}) + \boldW_s \boldx) 
%\otimes U)
%\label{eq:resnet}
%\end{equation}

\begin{figure}[]
	\includegraphics[width=\linewidth]{images/schematic/FPT}
	\caption{\label{fig:FPT} Function-preserving transformations used 
	to tranfer knowledge between the MotherNet and the ensembles.}
\end{figure}


%% Detailed explanation 

%\todo{In practice, how does the newly added parts of the filter change?}

%
%
%is applied such that 
%$\boldF_i = f \times f \times h$ 
%are applied to generate the output matrix $\boldW_{i+1} \in 
%\mathbb{R}^{(w-f+1) \times (h-f+1) \times k}$. 
%
%
%
%with spatial dimension 
%$w_i \times h_i$ and depth $d_i$. To generate layer $i+1$, output from 
%this layer is passed on to the next layer that has $k_i$ square filters 
%of spatial dimension $f_i \times f_i$ and depth $d_i$. If the size of 
%the stride is set to $1$, layer $i+1$ has spatial dimension $(w_i - f_i)+1 
%\times (h_i - f_i)+1$ and depth $k_i$. 
%%
%Net2WiderNet expands the filter size from $f_i \times f_i$ to 
%$f'_i \times f'_i$, where $f' = f + x$. For every depth of the 
%filter, the first $f_i \times f_i$ are the same 


% 

==> files/clustering.tex <==
\section{Analyzing Clustering}

\begin{itemize}
	\item The set of networks is $E = \{N_0, N_1, ..., N_{K-1}\}$.
	
	\item The edit distance between any two networks is $l(N_i, N_j)$. 
	
	\item Given a subset of these networks $S$, let $M_S$ be the 
	MotherNet for the subset. Let $\eta_S$ be the the sum of the 
	edit distances between $M_S$ and all networks in $S$ i.e., 
	$\eta_S = \sum_{i=0}^{|S|-1} l(M_S,S_i)$. In general, we 
	will use the notation of $\eta_{M,S}$ to be the sum of edit 
	distances between a MotherNet $M$ and a set of networks $S$. 
	 
	\item We want to explore what happens when we try to 
	create clusters by first ordering the networks based on 
	edit distances.
	
	\item First, we will construct $M_E$ i.e., the MotherNet 
	for all the networks in $E$. Then, we will reorder $E$ 
	based on the Levenshtein distance between $M_E$ and networks 
	in $E$ such that $l(M_E, N_{i}) \geq l(M_E, N_{i-1}) \forall 
	i$.
	
	\item Then, to create $g$ clusters, we will pick $g$ equi-sized 
	ordered subsets of $E$. 
	
	\td{There are a few things we can try to prove:}
	
	\item By doing this, we minimize the sum of edit distances 
	$\sum_{i=0}^{G-1} \eta_{C_i}$ between these MotherNets 
	constrained on having equi-sized clusters 
	
	\item Let $E_{1:K-1}$ be all networks in $E$ with the exception 
	of the first network $N_0$. 
	
	\td{Is $\eta_{E_{1:K-1}} \leq \eta_{E}$?}
	
	\item This should be true as $N_0$ can only have a non-negative 
	edit distance from $M_E$. Removing it cannot increase the 
	$\eta_{M_E, E_{1:K-1}}$ (sum of the edit distances from $M_E$ 
	to networks in $E_{1:K-1}$. Furthermore, $\eta_{E_{1:K-1}} \leq 
	\eta_{M_E, E_{1:K-1}}$, as $l(M_{E_{1:K-1}},E_i) \leq l(M_{E},E_i) 
	\forall i \in \{1,2,...,K-1\}$. 
	
	\item In other words, shrinking the subset from the left can 
	either reduce $\eta$ or $\eta$ remains the same.            
\end{itemize}

==> files/convNets.tex <==
%
\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{images/schematic/NN_example}
%	\vspace{0.1in}	
	\caption{Fundamentals of Neural Networks.}
	\label{fig:NN_example}
\end{figure}
%

% TODO Revise this section. 
\section{Neural Networks}

% Neural networks introduction
Neural networks are widely popular machine learning models 
that are loosely modeled after the neuronal structure of 
the mammalian cerebral cortex \cite{Caudill1987}. They are 
composed of one or more highly interconnected layers of units 
called neurons. Here, we provide some fundamental concepts 
related to neural networks with a focus on training.  
%

%
\boldPara{Neurons.} 
A neuron is the smallest building block of a neural network. 
Every neuron has an associated set of weights, a bias, and, 
optionally, an activation function. A neuron takes as input 
one or more neurons' output (or if the neuron is from the 
first hidden layer, it takes as input some region from within 
the input data item such as one or more pixels from an image) 
and computes an output. 
%
Figure \ref{fig:NN_example} shows examples of neurons 
($x_1,x_2,$ and $x_3$) depicted with dotted circles. 

%
\boldPara{Layers.} A layer in a neural network is composed of a set of 
neurons. The neurons in a certain layer interact with output from 
the previous layer. The output of this layer feeds into the next layer. 
In general, a neural network consists of an input layer, an output layer, 
and one or more hidden layers.
% 
Layers are shown as rectangles in Figure \ref{fig:NN_example}. 

%
\boldPara{Parameters.} These are a set of numeric weights that are 
associated with every neuron in the network. Typically, there is a 
weight for every input of the neuron and these weights are 
multiplied to the input neuron. 
%
In Figure \ref{fig:NN_example}, $w1$ and $w2$ are parameters 
multiplied with the output of neuron $x_1$ and $x_2$. 

%
\boldPara{Architecture.} The overall setting of a neural network 
-- the number of layers, neurons in each layer, type of layers 
etc. -- is referred to as its architecture. 

%%
%\boldPara{Hyperparameters.} These are tuning knobs of a ConvNet that are 
%specified during initialization of a ConvNet.  
%They can be associated with individual layers (for instance, the number 
%of neurons and the class of activation function) or they can be global 
%(for instance, optimization strategy).  

%%
%\boldPara{Volume.} Layers, parameters, and receptive fields can all be 
%three dimensional. \rev{We will use \textit{spatial extent} to refer to their 
%width and height in such cases.} 

%
\boldPara{Training.} A set of labelled inputs is provided to the 
neural network during training. Based on this labelled data set, 
the neural network iteratively adjust its weights to learn how to 
assign labels to other data items that it may not have encountered 
before. The training process is composed of a set of alternating 
forward and backward passes until a specified metric (usually 
prediction accuracy) converges. 

%
\boldPara{Forward pass.} Given an architecture and a set of 
parameters, forward pass refers to the process of executing a 
neural network from the input layer to the output layer. This 
proceeds by sequentially applying all parameters associated with 
every layer to the previous layer and feeding its output to the 
next layer. This process produces a prediction (output) given 
an input. 

%
\boldPara{Backward pass.} During the backward pass, based on the 
quality of the prediction, the weights associated with the neural 
network are adjusted. This usually involves some optimization 
method such as gradient descent. 

%
\boldPara{Testing.} During testing, a neural network is 
given a set of inputs that it has not encountered before i.e., 
they were not a part of the training set. 
The performance (accuracy) of the neural network on these inputs is 
then measured. This requires just a forward pass per input. 

%
\boldPara{Accuracy.} 
The accuracy of a trained neural network is defined as the proportion 
of correct predictions on a given data set. 
%
If accuracy on the testing data set is comparable to the accuracy 
on the training data set, then the neural network generalizes well. 
On the other hand, if the testing accuracy is much less than the 
training accuracy, then the neural network overfits to the training data 
set and does not generalize well. 



\section{Convolutional Neural Networks}
% Overview %%%
% Why? 
Convolutional neural networks (ConvNets) are a special class of 
neural networks that take into account the spatial and temporal 
structure present in various data sets such as images and natural 
language. They do so through characteristic layers known as 
convolutional layers. 
% Overview
Here, we provide some background about ConvNets. 



%
\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{images/schematic/convNets_example}	
	\caption{Convolutional neural networks are composed of 4 different 
	types of layers.}
	\label{fig:convnet_example}
\end{figure}
%

%%% Layers %%% 
\boldPara{Layers in ConvNets}
%
ConvNets are composed of four different types of layers: convolutional, 
RELU, pooling, and fully-connected. 
%
Typically a ConvNet begins with one or more sequence of alternating 
convolutional and RELU layers; each followed by one or more pooling 
layers. Toward the end, there are one or more fully-connected layers.  
%
Figure \ref{fig:convnet_example} shows an example of a ConvNet with one 
instance of every type of layer. We briefly describe each of these 
layers. 


\paraTitle{Convolutional layer.} 
% significance
This layer is the core building block of ConvNets. Every neuron in this 
layer operates on a small spatial (typically a square) receptive field 
that extends through the full depth of the layer before it. The receptive 
fields of different neurons can have overlap between them, which depends 
on the stride length. 
% Execution 
Every neuron in this layer computes the dot product between 
its receptive field and weights, producing a two-dimensional output 
layer. Typically, multiple layers of neurons are stacked one after the 
other producing one output depth per stack. 
%
In Figure \ref{fig:convnet_example}, the convolutional layer has 
neurons with square receptive field of size $2 \times 2$, strided 
with a stride length of one, and there are two stacks of such neurons. 
Overall, this produces an output layer with depth two.  
% Purpose
Neurons within the same stack share weights. Effectively, this allows 
the network to learn filters (one per stack of neurons) that activate 
(produce high output) when specific features are detected.

\paraTitle{RELU layer.} 
RELU (Rectified Linear Unit) is one of the most popular activation 
function for neural networks and it is defined as follows: 

\vspace{-0.25in}
\begin{equation}
	f(x) = max(0,x)
\end{equation}

The RELU layer applies this function to every element in its input 
layer keeping both the spatial dimension and the depth intact. 

\paraTitle{Pooling layer.} 
% Purpose
This layer reduces the spatial dimension of its input layer. 
% Execution
Given a pooling function, a stride length, and a spatial receptive 
field, the pooling layer operates independently on every depth of 
the input layer and applies the pooling function (usually a non-linear 
downsampling function such as max or sum) to every box of the given 
receptive field strided with the given stride length. 
Figure \ref{fig:convnet_example} shows a pooling layer having 
neurons with receptive field of size $2 \times 2$ and stride 
length of one. 

\paraTitle{Fully-Connected layer.} 
% Significance
One or more fully-connected layers appear toward the end of 
ConvNets. Every neuron in this layer is connected to every 
neuron in the previous layer. Each neuron has a set of 
associated weights (as many as the number of neurons in the 
previous layer). The output of the last fully-connected 
layer is typically a probability distribution over labels 
associated with the input data item. In Figure \ref{fig:convnet_example}, 
the last fully-connected layer has four neurons that each provide 
an output that maps to a probability distribution over four labels. 
% purpose

% TODO | Use the same terminology as the main paper.

% Revise this section as well
\section{Ensembles of Deep Neural Networks}
% What are ensembles? 
In an ensemble, deep neural networks with diverse architectures 
are trained on the same or overlapping sub-samples of a data set 
to perform the same task. 
Then, during inference, the classification or prediction 
made by every member of the ensemble is combined together.
%
Formally, let $D = \{(x_1,y_1), (x_2,y_2), $ $\dots (x_N,y_N)\}$ be a 
training data set, where each feature vector $x_i$ has a ground 
truth label $y_i$. In an ensemble, we have $M$ neural network models 
$\{ \theta_1, \theta_2,$$ \dots \theta_{M}\}$, each of these 
models corresponds to an architecture in $\{ A_1, A_2,$
$ \dots A_{M}\}$.  The  model $\theta_m$ is a 
mapping between $x$ to $P$ (i.e., $\theta_m: x \rightarrow P$), 
where $P$ is a distribution over the set of labels. 
To classify a new data item $x'\notin D$, predictions from 
every model $\theta_m$ are combined together using some 
combination function $C: 
\{ \theta_1, \theta_2,$$ \dots \theta_{M}\} \rightarrow P$. 
Typically, this combination happens by taking some weighted 
average of individual predictions or through majority 
voting \cite{Ju2017}. 

\boldPara{Effectiveness of Ensembles} 
There are various reasons as to why diverse ensembles 
outperform individual models: First, ensembles enrich the space 
of hypotheses that are considered and are representationally 
richer \cite{Domingos1999}. Second, when ensemble models are 
combined together, using some form of averaging, the variation 
in the models, which is an artifact of stochastic training and 
non-convex objective function is reduced \cite{Dietterich2000}. 

% TODO Make the last line of this paragraph more concrete. 

\boldPara{Diverse Ensembles.} 
Diversity between models -- i.e., uncorrelated errors is a key 
requirement for ensembles to boost accuracy \cite{Lee2015,Ju2017}. 
Intuitively, if we train multiple models that capture different 
aspects of the classification problem, only then can we combine 
their individual predictions to improve accuracy. 
A neural network model within the ensemble may differ from others 
in a combination of the following ways: 
(i) parameter initialization; 
(ii) batch of training data it encounters; and 
(iii) architecture of the neural network. 
These variations result in diverse models that yield predictions 
with uncorrelated errors. 
%


==> files/exp.tex <==
\section{Experimental Analysis} 
\label{sec:experiments}

\td{Rephrase the improvement in terms of reduction of error rate 
as opposed to the raw numbers.}

% Introduction
We show how MotherNets provide better training time-accuracy 
tradeoff than existing fast ensemble training approaches as well 
as navigates this tradeoff. 

%%% %%% %%% %%% %%% 
\begin{table*}
\centering
\caption{\rev{Ensembles used in our experiments.}\label{tbl:ens}}
\vspace{0.1in}
\begin{tabular}{lllll} 

	\hline	
	\textbf{Ensemble}& 
	\textbf{Description}& 
	\textbf{Param.}&
	\textbf{SE alternative}&
	\textbf{Param.}\\
	\hline
	\textbf{V5}&
	VGG $13$, $16$, $16A$, $16B$, and $19$ 
	& 682M & VGG-16 $\times$ 5 & 690M
	\\
	\textbf{D5} & \rev{2 variants of DenseNet-40 and 3 variants of DenseNet-100} 
	& 17M
	& DenseNet-60 $\times$ 5 & 17.3M 
	\\
%	& \cite{Huang2017a} & & & 
%	\\
%	& \rev{of DenseNet-100 \cite{Huang2017a}}
	\textbf{R10}&
	$2$ variants each of ResNet 20, 32, 44, 56, and 110 & 327M & R-56 $\times$ 10 
	& 350M\\ 
	\textbf{V25}&
	$25$ variants of VGG-$16$ & 3410M & VGG-16 $\times$ 25 & 3450M
	\\
	\textbf{V100}&
	$100$ variants of VGG-$16$ & 13640M & VGG-16 $\times$ 100 & 13800M
	\\
	\hline
\end{tabular}
\end{table*}
%%% %%% %%% %%% %%%

\boldPara{Baselines.} 
We compare against five ensemble training approaches: 
full data set (\textit{FD}), bootstrap aggregation 
(\textit{BA}), knowledge distillation (\textit{KD}), snapshot 
ensembling (\textit{SE}), and TreeNets (\textsl{TN}). 
% SE
To provide a fair comparison against SE (where ensemble 
networks are constrained to be identical) we allocate the 
same total number of parameters to SE as the diverse architecture 
ensembles we use for the rest of the approaches. 
%
TN is designed only for networks without skip-connections and is not 
applicable to ensembles of DenseNets and ResNets \cite{Lee2015}. 
We omit comparison with TN for such ensembles.
%
For all of these approaches across all experiments, we ensure 
that we reach test error rates reported in literature 
\cite{Huang2017,Lee2015}.

\td{Revise the mention of diversity metrics here based on 
whether or not we include them in the final submission.}

\boldPara{Evaluation metrics.} \rev{We evaluate the training cost, 
ensemble test accuracy, and diversity.} 
% Training cost
For the training cost, we report the 
wall clock time as well as the monetary cost (in USD) for training on 
four different cloud instances across two providers.  
% Test accuracy
For ensemble test accuracy, we tried out various ensemble 
inference methods -- ensemble-averaging, super learner,  and voting 
-- and found that the method we use does not make any significant 
difference in our comparison with other baselines.  
%
We report the test error rate under the widely used ensemble-averaging 
method \cite{Guzman2012,Guzman2014,Ju2017,Stefan2015,Van2007}. 
% Diversity
%\rev{We quantify the diversity of ensembles by reporting the average 
%disagreement measure (DM). DM is widely used to quantify the 
%pairwise diversity between any two classifiers \cite{Kuncheva2003}. 
%It is the ratio of observations on which one classifier is correct 
%and the other is incorrect to the total number of observations.}  
%% 
%\rev{To extend this metric to the case with $K$ classifiers, we 
%calculate the pairwise diversity for all pairs of classifiers 
%and report the average value of their pairwise diversity.}


%%%% %%% %%% %%% %%% 
%\begin{table}
%\centering
%\caption{Ensembles used in our experiments.\label{tbl:ens}}
%\begin{tabular}{ll} 
%
%	\hline	
%	\textbf{Ens.}& 
%	\textbf{Description} \\
%	\hline
%	\textbf{V5}&
%	VGG $13$, $16$, $16A$, $16B$, and $19$ 
%%	\cite{Simonyan2014}
%	\\
%	\textbf{D5} & 5 variants of DenseNet-40 
%%	\cite{Huang2017a} 
%	\\ 
%%	& \rev{of DenseNet-100 \cite{Huang2017a}}
%	\textbf{R10}&
%	$2$ variants each of ResNet 20, 32, 44,\\ 
%	&  56, and 110 
%%	\cite{He2016} 
%	\\
%	\textbf{V25}&
%	$25$ variants of $V16$\\
%	\hline
%\end{tabular}
%\end{table}
%%%% %%% %%% %%% %%% 

\td{Mention a more diverse D5 ensemble.}



%
\boldPara{Training setup.} 
We adopt stochastic gradient descent with a mini-batch size of 
$256$ and batch-normalization to train all networks. All weights 
are initialized by sampling from a gaussian distribution with 
zero mean and unit standard deviation. Training data is randomly 
shuffled before every training epoch. 
%
The learning rate is set to $0.1$ for all experiments with the 
exception of DenseNets, where we use a learning rate of $0.1$ to train 
the MotherNets and $0.01$ to train hatched networks. This is inline 
with the learning rate decay used in the DenseNets paper 
\cite{Huang2017a}. {The same early stopping criterion is used across 
all networks and approaches: We stop training if the training 
accuracy does not improve within 15 epochs.} For snapshot 
ensembles, we use the optimal training hyperparameters as described 
in the paper: We set the initial learning rate $\alpha_0$ to 0.2 and 
train every snapshot for $60$ epochs \cite{Huang2017}.
%
%All experiments are run on the same server with Nvidia Tesla 
%V100 GPU. 


\td{Add description of D5}. 

\boldPara{Ensemble networks.} 
We experiment with ensembles of various convolutional architectures 
such as VGGNets, ResNets, and DenseNets. 
%
\rev{Ensembles of these architectures have been extensively used 
to evaluate fast ensemble training approaches \cite{Huang2017,Lee2015}.} 
%
Each of these ensembles are composed of networks having diverse 
architectures as summarized in Table \ref{tbl:ens}: 
%
$V5$ is composed of the 5 VGGNets described in the VGGNet paper 
\cite{Simonyan2014}. 
%
$R25$ contains ResNet architectures having a large difference 
in number of layers. 
%
$V25$ and $V100$ contain $25$ and $100$ variants of VGG-16 
respectively. All these networks have a distinct architecture 
and are created by varying one layer from VGG16 in one of three 
ways: (i) increasing the number of filters, (ii) increasing the 
filter size, or (iii) applying both (i) and (ii). 
%
To provide a fair comparison with SE (where the snapshots have to 
be from the same network architecture), we create snapshots as 
summarized in Table \ref{tbl:ens}.}

\boldPara{Data sets.} \rev{We evaluate on SVHN, CIFAR-10, 
and CIFAR-100 data sets \cite{Krizhevsky2009,Netzer2011}. 
%
The SVHN data set is composed of images of house numbers and 
has ten class labels. There are a total of $99$K images. We 
use $73$K for training and $26$K for testing. 
%
CIFAR-10 and CIFAR-100 data sets have $10$ and $100$ class 
labels respectively corresponding to various objects. There 
are a total of $60$K images -- $50$K training and $10$K 
testing images.} 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% %%% %%% V5 and D5 %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% 
\begin{figure*}[t!]
\captionsetup{width=\textwidth}
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/V5_tradeoff_full.pdf}
		\captionsetup{width=\textwidth}
		\caption{\rev{V5 (CIFAR-10)}}
		\label{exp:V5_all}
	\end{subfigure}
%	
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/V5_CIFAR10_training_time.pdf}
		\captionsetup{width=\textwidth}
		\caption{{Time breakdown (V5 C10)}}
		\label{exp:V5_CIFAR10_training_time}		
	\end{subfigure}
%		
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/D5_tradeoff.pdf}
		\captionsetup{width=\textwidth}
		\caption{\rev{D5 (CIFAR-10)}}
		\label{exp:Dense5_all}
	\end{subfigure}
%	
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/D5_CIFAR10_training_time.pdf}
		\captionsetup{width=\textwidth}
		\caption{\rev{Time breakdown (D5 C10)}}
		\label{exp:Dense5_CIFAR10_training_time}
	\end{subfigure}
%
	\caption{In comparable training time, MotherNets 
	achieve significantly better accuracy ($1$ to $2.5$ 
	percent lower test error) than state-of-the-art fast ensemble 
	training approaches.}
\end{figure*}
%%%% %%% %%% V5 and D5 %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Better training time-accuracy tradeoff} 
We begin our evaluation with two ensembles of five networks 
each -- V5 and D5 from Table \ref{tbl:ens} -- trained on the 
CIFAR-10 data set. 
%
For SE we train a comparable ensemble of five identical 
networks: For V5 ($682$M parameters), we compare against an ensemble 
of five V16 ($690$M parameters), whereas for D5 ($17$M parameters), we compare 
against an ensemble of five DenseNet-60 ($17.3$M parameters). 
%
For TN, we varied the number of shared layers and found that 
sharing $3$ out of $16$ layers provides the best accuracy. This 
is similar to the optimal proportion of shared layers in the 
TreeNets paper \cite{Lee2015}. 
%

Figure \ref{exp:V5_all} and Figure \ref{exp:Dense5_all} plot accuracy 
(test error rate) against training time achieved by all approaches 
for V5 and D5 respectively. 
%
The horizontal lines indicate the accuracy of single VGGNet and 
DenseNet model on CIFAR-10 \cite{Hasanpour2016,Huang2017a}. 
%
In both figures, points closer to the y-axis 
train faster, whereas those near the x-axis provide better accuracy.  
%
As we vary the number of clusters $g$, MotherNets navigate this 
tradeoff from being training time-optimized (at $g=1$) to 
accuracy-optimized (at $g=5$). As $g$ approaches five, MotherNets 
is similar to FD, where all networks are independently trained 
using the entire data set with random parameter initialization. 



% Figures: 
%Figure \ref{exp:V5_all} shows the ratio of accuracy (test error rate) 
%to training time achieved by all approaches. In Figure \ref{exp:V5_all}, 
%points closer to the y-axis train faster, whereas those near the x-axis 
%provide better accuracy.  
%%
%As we vary the number of clusters $g$, MotherNets navigate this 
%tradeoff from being training time-optimized (at $g=1$) to 
%accuracy-optimized (at $g=5$). As $g$ approaches five, MotherNets 
%is similar to FD, where all networks are independently trained 
%using the entire data set with random parameter initialization. 
%%
%The horizontal line indicates state-of-the-art accuracy of a 
%single VGGNet model on CIFAR-10 \cite{Hasanpour2016}. 

%\cmt{We will incorporate DenseNet results here.}

% Observations
For both ensembles, we observe that time-optimized MotherNets 
achieve an overall better accuracy-training time tradeoff i.e., 
MotherNets is both faster and more accurate than KD, TN, and 
BA\footnote{We omit BA from all our tradeoff graphs 
(Figure \ref{exp:V5_all}, Figure \ref{exp:Dense5_all}, 
Figure \ref{exp:R_25_CIFAR_10_tradeoff}, 
Figure \ref{exp:V_25_CIFAR_100_tradeoff}, and 
Figure \ref{exp:V_25_SVHN_tradeoff}) as it is a clear outlier: 
It takes on average $73$ percent of the time to train as compared 
to FD but still results in significantly higher test error rate 
than any of the baseline approaches including the single model. 
This is because BA reduces the number of unique data items seen 
by individual models and is ineffective when training 
highly parameterized models such as neural networks 
\cite{Domingos1999,Lee2015}.}.
% Explanation of the trends:
The low error rate stems from the fact that transferring the learned 
function from the MotherNet to the ensemble networks provides a good 
starting point as well as {introduces regularization for further 
training.} This reduces both the bias and the variance of the ensemble 
(e.g., for V5 around $5\times$, $4\times$, and $4.1\times$ faster 
than FD, KD, and BA respectively) requiring less overall training time as 
shown in Figure \ref{exp:V5_CIFAR10_training_time} and Figure 
\ref{exp:Dense5_CIFAR10_training_time}. 
%

% KD
MotherNets significantly outperform KD in both accuracy and training 
time. The lower accuracy of KD stems from the fact that all ensemble 
networks are more closely tied to the base network as they are trained 
from the output of the same network. The higher training cost is because 
distilling a network still takes around $60$ to $70$ percent of the 
time required to train from scratch.
%
%
TreeNets provide similar accuracy to MotherNets with $g=1$ but 
takes around $3 \times$ longer to train. This is because the 
per epoch cost is higher and it takes multiple epochs to converge. 
In the same time budget, MotherNets can train with $g=4$ providing over 
one percent lower test error rate.

% SE
The training time for SE and MN (with $g=1$) are comparable: SE takes 
60 epochs to train one snapshot, whereas MotherNets takes 128 epochs 
to train individual MotherNets and on average 40 epochs to train each 
ensemble network. MotherNets provide better accuracy for V5 -- 
around $0.7$ percent lower test error rate for $g=1$ and around 
$1.25$ percent lower test error rate for $g=2$. \rev{For the D5 
ensemble, SE lies in between MotherNets with $g=1$ and $g=2$. 
For a little decrease in accuracy, MotherNets with $g=1$ can train 
around $10$ percent faster or provide $0.5$ percent better accuracy 
if given $40$ percent more training time with $g=2$.} 



%Figure \ref{exp:V5_CIFAR10_training_time} shows the training 
%time split between different ensemble networks across different 
%approaches.

%\boldPara{Accuracy-training time tradeoff.} 
%\rev{While the accuracy of MotherNets (with a single cluster) is 
%slightly lower than FD, however, MotherNets strike a much better 
%accuracy-training time balance reaching the same accuracy 
%significantly faster. This is depicted in Figure 
%\ref{exp:V5_CIFAR10_tradeoff}, which shows the percentage test 
%error rate on the x-axis and the time taken to reach it on 
%the y-axis. 
%%
%%Figure \ref{exp:vary_clusters} shows the accuracy and training 
%%time of MotherNets with different number of clusters. 
%%
%Overall, we observe that MotherNets provide a non-linear 
%accuracy-training time tradeoff i.e., we can save a lot of 
%time while not losing so much in accuracy as compared to 
%full-data. For instance,  we can achieve X percent of the 
%final accuracy with only Y percent of FD's training time. 
%Furthermore, we can tune this tradeoff by varying the number 
%of clusters (i.e., tuning the clustering parameter $\tau$). } 

%Further, MotherNets strike a much better accuracy-training time 
%balance than any of the existing approaches reaching the same 
%accuracy significantly faster. This is depicted in Figure \ref{exp:V5_CIFAR10_tradeoff}, which shows the percentage test 
%error rate on the x-axis and the time taken to reach it on the 
%y-axis. We omit bagging and knowledge distillation from this 
%graph as their final accuracies are not comparable to MotherNets 
%and full-data.
%%
%{Figure \ref{exp:vary_clusters} shows the accuracy and training 
%time of MotherNets with different number of clusters. 
%%
%Overall, we observe that MotherNets achieve a non-linear accuracy-training 
%time tradeoff i.e., we can save a lot of time while not losing so 
%much in accuracy as compared to full-data. Furthermore, we can tune 
%this tradeoff by varying the number of clusters (i.e., tuning the 
%clustering parameter $\tau$).} 

%% %%% %%% %%% %%% 
\begin{figure*}[t!]
% R10 C10
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/R_10_CIFAR_10_tradeoff.pdf}
		\caption{\rev{R10 (CIFAR-10)}}
		\label{exp:R_25_CIFAR_10_tradeoff}
	\end{subfigure}
% V25 C100
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/V_25_CIFAR_100_tradeoff.pdf}
		\caption{V25 (CIFAR-100)}
		\label{exp:V_25_CIFAR_100_tradeoff}
	\end{subfigure}
% V25 SVHN
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/V_5_SVHN_tradeoff.pdf}
		\caption{\rev{V25 (SVHN)}}
		\label{exp:V_25_SVHN_tradeoff}
	\end{subfigure}
	% Cloud cost
	\begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]
			{images/experiments/revised/V_100_CIFAR10.pdf}
		\caption{\rev{V100 (CIFAR-10)}}
		\label{exp:V_100_CIFAR_10_tradeoff}
	\end{subfigure}
%% Cloud cost
%	\begin{subfigure}{0.245\textwidth}
%		\includegraphics[width=\textwidth]
%			{images/experiments/revised/training_cost.pdf}
%		\caption{\rev{Training cost (USD)}}
%		\label{exp:training_cost}
%	\end{subfigure}
%
\caption{\rev{MotherNets strike a better accuracy-training time 
tradeoff than existing fast ensemble training approaches when 
training large ensembles of neural networks across different data 
sets.}}
\end{figure*}
%% %%% %%% %%% %%% 

%%%% %%% %%% %%% %%% 
%\begin{figure*}[t!]
%\captionsetup{width=0.49\textwidth}
%% TODO E | Why low improvement? 
%%\begin{minipage}{0.495\textwidth}
%%	\begin{subfigure}{0.495\textwidth}
%%		\includegraphics[width=\textwidth]
%%		{images/experiments/vote_V_large_SVHN}
%%		\caption{Ensemble test error rate}
%%	\end{subfigure}
%%	\begin{subfigure}{0.495\textwidth}
%%		\includegraphics[width=\textwidth]
%%		{images/experiments/V_large_SVHN_training_time}
%%		\caption{Ensemble training time}
%%	\end{subfigure}
%%	\caption{Ensemble of 50 VGGNets (SVHN)}
%%	\label{exp:V_large_SVHN}
%%\end{minipage}
%% TODO E | Bagging and MN to close by.
%\begin{minipage}[t]{0.49\textwidth}
%	\begin{subfigure}[t]{0.49\textwidth}
%		\includegraphics[width=\textwidth]
%%		{images/experiments/v_large_CIFAR100}
%		{images/experiments/vote_R_large_CIFAR10}
%		\caption{Ensemble test error rate}
%	\end{subfigure}
%	\begin{subfigure}[t]{0.49\textwidth}
%		\includegraphics[width=\textwidth]
%		{images/experiments/R_large_CIFAR10_training_time}
%		\caption{Ensemble training time}
%	\end{subfigure}
%	\caption{Ensemble of 25 ResNets (CIFAR-10)}
%	\label{exp:R_large_CIFAR10}
%\end{minipage}
%\begin{minipage}[t]{0.2375\textwidth}
%		\captionsetup{width=0.9\textwidth}
%		\includegraphics[width=\textwidth]
%		{images/experiments/compare_all_.pdf}
%		\caption{Comparing accuracy of MotherNets, 
%		full-data, and bagging.}
%		\label{exp:compare_all}
%\end{minipage}
%\begin{minipage}[t]{0.2375\textwidth}
%		\captionsetup{width=0.9\textwidth}
%		\includegraphics[width=\textwidth]
%		{images/experiments/mixed_CIFAR10_training_time.pdf}
%		\caption{Ensemble of diverse architecture classes.}
%		\label{exp:mixed_CIFAR10_accuracy}
%\end{minipage}
%\vspace{-0.2in}
%\end{figure*}
%%%% %%% %%% %%% %%% 

\td{Combine the two experiments under this section together.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Scaling ensemble and data size} 
Next, we show how MotherNets exhibit a superior 
accuracy training-time tradeoff as we scale the 
complexity and size of the ensemble as well as 
the data sets.

\td{Possibly add how accuracy scales for R10C10.}

\boldPara{R10 on CIFAR-10.}
First, we present results on R10 from Table \ref{tbl:ens} trained 
on the CIFAR-10 data set. This ensemble consists of networks with large 
size differences.
%
We compare against SE, KD, BA, and FD. For SE, we train an ensemble of 
10 ResNets-56 having comparable parameters to R10. 
%TN is designed 
%for networks without skip-connections and as such it is not applicable 
%in this scenario \cite{Lee2015}.

We observe that training time-optimized MotherNets (at $g$ = 1)
outperforms all other approaches. In particular MotherNets provide 
a better training time-accuracy tradeoff than SE. This is because 
the test accuracy of SE shows diminishing return as we increase 
the number of snapshots. This trend is also observed in the 
Snapshot paper \cite{Huang2017}.
%
Overall, MotherNets establish a new baseline for ResNet ensembles 
on CIFAR-10 achieving below {4.5} percent test error rate in 
the same time SE achieves around 5.1 percent \cite{He2016,Huang2017}.



\boldPara{V25 on CIFAR-100 and SVHN.} 
% 
Next, we experiment with $V25$ from Table \ref{tbl:ens}.  
%
All 25 networks have a distinct architecture and are created by 
varying one layer from VGG16 in one of three ways: (i) increasing 
the number of filters, (ii) increasing the filter size, or 
(iii) applying both (i) and (ii). 

Figure \ref{exp:V_25_CIFAR_100_tradeoff} and Figure 
\ref{exp:V_25_SVHN_tradeoff} show the ratio of accuracy 
to training time achieved by MotherNets on the CIFAR-100 
and the SVHN data sets respectively. 
%
\rev{For the CIFAR-100 data set, MotherNets ($g=1$) provide over $1.5$ 
percent lower test error rate than SE in comparable training time. 
For this data set, SE is unable to even improve upon the accuracy 
of a single VGGNet model trained from scratch. 
%
For the SVHN data set, SE provides better accuracy than MotherNets 
($g=1$). However, MotheNets ($g=2$) results in comparable accuracy 
in around the same amount of training time as SE.} 

%
For all ensemble training approaches, the improvement in accuracy 
over a single model for CIFAR-100 (around 5 percent) is much higher 
than it is for CIFAR-10 or SVHN. This is inline with theoretical 
frameworks, which postulate that data sets with more labels benefit more 
from large ensembles \cite{Bonab2016,Bonab2017,Oshiro2012} and MotherNets 
enable this by rapidly training very large ensembles. 

\boldPara{V100 on CIFAR-10.} \rev{Next we present results on an 
extremely large ensemble of $100$ VGGNets. Figure 
\ref{exp:V_100_CIFAR_10_tradeoff} shows how training time 
optimized MotherNets ($g=1$) compares with SE. We observe 
that as we increase the number of networks in an ensemble, 
the training time of MN grows at a much smaller rate than 
that of SE. Furthermore, ensembles trained through MotherNets 
continues to improve in accuracy, whereas SE actually gets 
worse as we increase the number of snapshots. This declining 
accuracy as the size of the ensemble increases is in line 
with the Snapshot paper \cite{Huang2017}.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Scaling ensemble and data size} 
%Next, we show how MotherNets exhibit a superior accuracy training-time 
%tradeoff as we scale the complexity and size of the ensemble as well 
%as the data sets.
%
%\td{Possibly add how accuracy scales for R10C10.}
%
%\boldPara{R10 on CIFAR-10.}
%First, we present results on R10 from Table \ref{tbl:ens} trained 
%on the CIFAR-10 data set. This ensemble consists of networks with large 
%size differences.
%%
%We compare against SE, KD, BA, and FD. For SE, we train an ensemble of 
%10 ResNets-56 having comparable parameters to R10. 
%%TN is designed 
%%for networks without skip-connections and as such it is not applicable 
%%in this scenario \cite{Lee2015}.
%
%We observe that training time-optimized MotherNets (at $g$ = 1)
%outperforms all other approaches. In particular MotherNets provide 
%a better training time-accuracy tradeoff than SE. This is because 
%the test accuracy of SE shows diminishing return as we increase 
%the number of snapshots. This trend is also observed in the 
%Snapshot paper \cite{Huang2017}.
%%
%Overall, MotherNets establish a new baseline for ResNet ensembles 
%on CIFAR-10 achieving below \rev{3.5} percent test error rate in 
%the same time SE achieves around 5 percent \cite{He2016,Huang2017}.
%
%
%
%\boldPara{V25 on CIFAR-100 and SVHN.} 
%% 
%Next, we experiment with $V25$ from Table \ref{tbl:ens}.  
%%
%All 25 networks have a distinct architecture and are created by 
%varying one layer from VGG16 in one of three ways: (i) increasing 
%the number of filters, (ii) increasing the filter size, or 
%(iii) applying both (i) and (ii). 
%
%Figure \ref{exp:V_25_CIFAR_100_tradeoff} and Figure 
%\ref{exp:V_25_SVHN_tradeoff} show the ratio of accuracy to training 
%time achieved by MotherNets on the CIFAR-100 and the SVHN data sets 
%respectively. 
%%
%Overall, MotherNets continues to dominate other fast ensemble 
%training approaches. SE performs somewhat inconsistently across 
%different architectures and data sets. For instance, it provides 
%a competitive training time-accuracy tradeoff to MotherNets for 
%the SVHN data set but is unable to achieve state-of-the-art 
%accuracy of a single VGGNet model for CIFAR-100.  
%%
%For all ensemble training approaches, the improvement in accuracy 
%over a single model for CIFAR-100 (around 5 percent) is much higher 
%than it is for CIFAR-10 or SVHN. This is inline with theoretical 
%frameworks, which postulate that data sets with more labels benefit more 
%from large ensembles \cite{Bonab2016,Bonab2017,Oshiro2012} and MotherNets 
%enable this by rapidly training very large ensembles. 




\td{Maybe add an experiment with different architecture 
classes D50 maybe.}

\td{Maybe add an experiment that demonstrate why diversity in 
architecture is a good thing.}


\subsection{Improving training cost} 
Now, we show how the improvement in training time achieved by 
MotherNets translates into USD amount saving when training 
on the cloud. Figure \ref{exp:training_cost} shows the cost (in USD) 
of training on four cloud instances across two cloud service 
providers: 
(i) M1 that maps to AWS P2.xlarge and Azure NC6, and 
(ii) M2 that maps to AWS P3.2xlarge and Azure NCv3. M1 is priced 
at USD $0.9$ per hour and M2 is priced at USD $3.06$ per hour 
for both cloud service providers 
\cite{awsPricing,azurePricing}. 

\rev{Across both of these machines, training time-optimized MotherNets 
provide significant reduction in training cost (up to $3 \times$) as 
it can train a very large ensemble in a fraction of the training time 
as compared to other approaches.} 
%
Overall, it is more cost-effective to train on M2 as compared 
to M1. This is because despite being $3\times$ more expensive 
per unit time, M2 is on average (taken over our experiments) 
$8.6 \times$ faster than M1. 
%


\td{Why do fewer parameters improve inference time?}

\begin{wrapfigure}{r}{0.25\textwidth}
		\includegraphics[width=0.25\textwidth]
			{images/experiments/revised/training_cost.pdf}
		\caption{\rev{Training cost (USD)}}
		\label{exp:training_cost}
		\vspace{-0.15in}
\end{wrapfigure}
\boldPara{Improving inference time.} 
\rev{Figure \ref{exp:V5_inference} shows how {shared-MotherNets} 
improves inference time for V5 trained on the CIFAR-10 data set. 
We report both overall ensemble test error rate and the inference 
time per image across various number of clusters. We see up to 
$2 \times$ improvement in inference time with negligible loss 
in accuracy. This is because shared-MotherNets has a reduced 
number of parameters requiring less computation. This improvement 
scales with the ensemble size. 
%
As the number of clusters increase, so does the number of separate 
networks we have to infer from. This leads to a scenario, where at 
$g=5$, Shared-MotherNets is equivalent to MotherNets both in 
terms of inference time and accuracy.} 




==> files/infer.tex <==
\section{Efficient Ensemble Inference}

\boldPara{Introductory paragraph.} 

\begin{itemize}
	\item Here we explain how MotherNets improves the inference 
	efficiency of ensembles by training and maintaining a single 
	copy of parameters that originate from the MotherNet. 
\end{itemize}

\boldPara{Constructing shared MotherNet.} 

\begin{itemize}
	\item This happens during the incremental training phase. 
	\item The overall idea is to create a network structure 
	from the ensemble specification and the trained MotherNet 
	in which parameters of the trained MotherNet are completely 
	shared. 
	\item One way of doing it is by first applying 
	function-preserving transformations to the trained MotherNet 
	and get all of the ensemble networks. After that is done, we 
	go through the ensemble networks, concatenating the input 
	to the MotherNet layers and diverging them from there onwards. 
\end{itemize}



 

==> files/intro_inference.tex <==
\section{Introduction}

\begin{figure*}[t!]
	\includegraphics[width=\linewidth]{images/schematic/example}
	\caption{\label{fig:example} MotherNet accelerates the training 
	of neural network ensembles.}
	\vspace{-0.2in}
\end{figure*}

% 

%\cmt{I am not quite thrilled about two approaches being mentioned 
%side-by-side.}


\boldPara{Neural network ensembles.} 
Ensembles of deep neural networks with diverse architectures 
trained on the same data set have been shown, both theoretically 
and empirically, to improve generalization accuracy 
\cite{Dietterich2000,Drucker1993,Granitto2005,Ju2017,
Stefan2015,Russakovsky2015,Xu2014}.
% 
For instance, by combining several image classification 
convolutional networks, the generalization accuracy on 
the CIFAR-10 data set improves by up to three percent \cite{Ju2017}.
%
Further, most of the winners and top performers on the ImageNet 
challenge are ensembles of deep neural networks 
\cite{Stefan2015,Russakovsky2015}. 
% 
However, training \rev{and deploying} ensembles of many deep neural 
networks takes a prohibitively large amount of time and 
computational resources. 
%
For instance, even on high performance hardware, training 
a single deep neural network can take up to a few days to 
complete \cite{Huang2017}. 
This cost grows linearly with the size of the ensemble 
as every neural network added to the ensemble needs to 
be first trained \rev{and then, during deployment, 
inferred from}. 

% 
\boldPara{Restrictive ensemble size.} Because 
of this prohibitive training \rev{and deployment} cost, 
researchers and practitioners 
can only feasibly train and \rev{deploy} small ensembles with a 
few different deep neural network architectures 
\cite{He2016,Huang2017a,Huang2017,Szegedy2015}. 
%
Specifically, neural network ensembles have a much smaller size 
when compared with ensembles of other algorithms. 
For instance, random forest, a popular ensemble 
algorithm, may contain hundreds of individual models (decision 
trees), whereas ensembles of neural networks consist of five 
to ten models 
\cite{He2016,Huang2017a,Huang2017,Oshiro2012,Szegedy2015}. 
%
This is restrictive since theoretical frameworks 
suggest that the generalization accuracy of an ensemble 
increases with the number of well-trained models it 
contains \cite{Bonab2016,Bonab2017,Oshiro2012}. 
%
This trend continues at least until the ensemble size becomes 
equal to class labels (of which there could be thousands in 
state-of-the-art classification systems) \cite{Bonab2016,Bonab2017}. 
% 

%
\boldPara{Slow ensemble training.} 
Existing approaches to train ensembles of deep neural networks 
with different architectures fall under two distinct categories: 
%
(i) training every network architecture using the entire data set 
with random parameter initialization \cite{Huang2017,Ju2017,Stefan2015}, 
and 
%
(ii) training every network architecture using a different subset 
sampled with replacement from the original data set (e.g., bagging 
or boosting) \cite{Stefan2015,Moghimi2016}. 
%
Since deep neural networks have a large parameter space, training 
with the full data set is required to achieve low bias 
\cite{Huang2017,Ju2017,Stefan2015}, however it takes more time. 
Of the sub-sampling approaches, bagging may converge faster but 
results in higher bias as it effectively trains the neural 
networks with less unique data items \cite{Domingos1999}. 
Boosting on the other hand, can result in good accuracy but has 
been shown to overfit and is inherently hard to parallelize 
\cite{Moghimi2016}. In terms of training cost, all of these 
approaches still train every network from scratch and require 
a significant amount of time and computational resources. 

\boldPara{Expensive ensemble deployment.} \rev{Once ensembles of neural 
networks are trained, deploying them requires substantially more 
computational resources (as compared to a single model) and can 
drastically slow down the inference process. This is because to 
make even a single decision, for instance classifying an image, we 
need to run the complete inference process for every neural network 
in the ensemble and then combine the results.}  

%%% %%% %%%
\begin{wrapfigure}{R}{0.18\textwidth}
\includegraphics[width=0.18\textwidth]{images/schematic/concept}
\caption{\label{fig:concept}MotherNet vs. existing ensemble training approaches.
}
\vspace{-0.05in}
\end{wrapfigure}
%%% %%% %%%


% 
\boldPara{MotherNets.}
We propose MotherNets that enable rapid training \rev{and efficient 
deployment} of very large ensembles of neural networks with 
different sizes and architectures. \rev{The main idea is to capture 
the structural similarity that exists between members of a neural 
network ensemble. Then, during training, train for it once, and 
during deployment, infer from it once.}

\boldPara{Rapid training.} 
%
Through MotherNets we can train an ensemble significantly faster 
than approaches that train on sub-samples of the data, while 
achieving generalization accuracy comparable to that of training 
with the full data set. Conceptually, the relationship between 
MotherNets and existing training approaches is shown in Figure 
\ref{fig:concept}. 
%
To achieve this improvement in training cost we train ensembles 
of neural networks as follows: Given an ensemble of feed-forward 
neural networks, we construct the MotherNet, which captures 
the structural similarity between all of the ensemble networks 
(Figure \ref{fig:example}a). 
%
This MotherNet is then trained once using full data set to 
achieve low bias (Figure \ref{fig:example}b). 
%
Once the MotherNet is trained, every network in the ensemble 
can be \textit{hatched} from it using function-preserving 
transformations that ensure knowledge from the MotherNet is exactly 
transferred to every network of the ensemble \cite{Chen2015,Wei2016} 
(Figure \ref{fig:example}c). 
The ensemble networks are then trained, 
%using bootstrap aggregation 
converging significantly faster (typically in a few tens of epochs) 
as compared to training from scratch. 

\boldPara{Efficient deployment.} \rev{MotherNets improves the 
efficiency of deploying ensembles of neural networks reducing 
both the inference time and memory requirement. 
%
To achieve this, during incremental training (Figure \ref{fig:concept}c), 
we jointly train parameters originating from the MotherNet instead of 
training these parameters separately in the ensemble networks. Then, 
during deployment, this saves memory as we have to maintain only one 
jointly trained copy of the MotherNet parameters instead of one for 
each ensemble network. 
Similarly, the inference time is reduced because we have to do a 
single pass over MotherNet parameters and only incremental passes 
over the rest of the parameters in the ensemble networks.}




This brings distinct benefits: 
(i) As the size of the ensemble grows, the training \rev{and 
inference} time grows at a much lower rate than that of existing 
approaches. This is because every additional network can be hatched 
from the trained MotherNet and trained significantly faster as 
compared to training from scratch. Practically, this allows us 
to use -- train and deploy -- very large ensembles of deep neural 
networks.  
%
(ii) MotherNets ensures that both the bias and the variance of the 
ensemble is low. This is because the MotherNet is trained using the 
entire data set achieving low bias, which is then transferred to the 
ensemble networks that are trained using sub-sampling approaches 
that both reduce variance as well as explicitly create diversity 
\cite{Domingos1999}. 
%


% Results
\boldPara{Results.} 
We show through experiments that MotherNets can \rev{substantially 
reduce training and inference time for ensembles of diverse 
neural networks} on CIFAR-10, CIFAR-100, and SVHN data sets. 
%
{In particular, we show that in time taken to train an 
ensemble of $15$ networks using existing approaches, we can 
train an ensemble of up to $100$ networks that continue to 
improve generalization accuracy.} 
%
In addition, our results show 
that the overall improvement in training time (relative to 
existing approaches) increases with the ensemble size. 
%




==> files/main.tex <==
\section{Training ensembles through MotherNets}

First, we define the MotherNet and then explain how we use it 
to train an ensemble of neural networks. 

\boldPara{MotherNet.} 
Given an ensemble with different neural network architectures, the 
MotherNet captures the largest structural similarity 
between the ensemble networks. 
Formally, it is the largest neural network from which 
members of an ensemble can be obtained by applying a sequence of 
function-preserving transformations. Function-preserving 
transformations allow us to expand the size of a trained network, 
while preserving its function \cite{Chen2015,Wei2016,Wei2017}. 
Given an ensemble, many neural networks with size less than all 
of the ensemble networks can be expanded through function-preserving 
transformations to obtain the ensemble networks. 
The MotherNet is defined to be the largest of such networks. It 
follows from this definition that: 
(i) ensemble networks hatched from the MotherNet can immediately 
inherit its function (mapping between input data items and output 
labels) and 
(ii) the structure of the MotherNet is smaller than or equal to the 
ensemble network with the smallest size. 


\boldPara{Function-preserving transformations.} 
We provide a brief overview of function-preserving transformations. 
They allow us to grow the size of a neural network, while ensuring 
that the function it represents is preserved. 
%
Function-preserving transformations enable the 
ensemble networks to \textit{inherit} the learnt function from 
the MotherNet. 
%
We use three classes of function-preserving transformations 
as shown in Figure \ref{fig:FPT} and they allow us to increase the 
depth of the network (Figure \ref{fig:FPT}a), widen the network 
layers (Figure \ref{fig:FPT}b), and grow the size of convolutional 
filters (Figure \ref{fig:FPT}c). 
% 
There are two distinct approaches to achieve these transformations: 
Net2Net and Network Morphism. 
%
Net2Net increases the capacity of the given network by adding identity 
layers or by replicating existing weights \cite{Chen2015}. 
%
Network Morphism, on the other hand, derives sufficient and necessary 
conditions that when satisfied will extend the network while preserving 
its function and provides algorithms to solve for those conditions 
\cite{Wei2016,Wei2017}. 
%
In MotherNet, we adopt the second approach 
\footnote{There is ongoing research on function-preserving 
transformations. Novel and better approaches introduced in 
the future can also be applied within the context of 
MotherNets.} 
i.e., Network Morphism, as 
it has been shown to serve as a better starting point for further 
training of the expanded network as compared to Net2Net \cite{Wei2016,Wei2017}. 
These 
transformations are readily applicable to a wide range of feed-forward 
neural networks including VGGNets, ResNets, and 
DenseNets \cite{Chen2015,Wei2016,Wei2017}.
%



\begin{figure*}[]
	\includegraphics[width=\linewidth]{images/schematic/FPT}
	\caption{\label{fig:FPT} MotherNet uses three function-preserving 
	transformations to hatch ensemble networks.}
	\vspace{-0.175in}
\end{figure*}


%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
\subsection{Constructing the MotherNet}

First, we provide a method to construct the MotherNet $M$ from 
an ensemble $E = \{N_0, N_1, \dots N_{K-1}\}$ of $K$ neural 
networks (where $N_k$ denotes a neural network architecture 
in the ensemble). 
%
We describe how to construct $M$ for ensembles of both 
fully-connected and convolutional neural networks. 
%
%Then, we explain how we handle the case 
%where networks in the ensemble have a large difference in size. 

%% Fully-connected Networks
\textbf{Fully-connected networks.} 
For ensembles of fully-connected neural networks, $M$ is 
constructed as follows: First, its input and output layers 
have the same structure as all the networks in $E$, since 
they are all trained for the same task. Then, $M$ is 
initialized with as many hidden layers as the shallowest 
network in $E$.  
% 
Then, we construct the hidden layers of $M$ one-by-one going from 
the input to the output layer such that the structure of the $i$-th 
hidden layer of $M$ is the same as the $i$-th hidden layer of the 
network in $E$ with the least number of parameters. 


Figure \ref{fig:example}a depicts an example of an ensemble, 
with two three-layered networks and one four-layered network, 
where the MotherNet consists of three layers. 
%
Every layer of the MotherNet is constructed such that it 
has the same structure as the layer with the least number of parameters 
at that position (shown in bold in Figure \ref{fig:example}a). 

\textbf{Convolutional neural networks.}  
%
Convolutional neural network architectures consist of blocks of 
convolutional layers separated by max-pooling layers 
\cite{He2016,Shazeer2017,Simonyan2014,Szegedy2015}. 
These blocks are then followed by another block of one or more 
fully-connected layers.
For instance, VGGNets are composed of five blocks of convolutional 
layers separated by max-pooling layers, whereas, DenseNets consist 
of four blocks of densely connected convolutional layers. 
%
For such networks, we construct the MotherNet $M$ 
block-by-block instead of layer-by-layer. 
The intuition is that deeper or wider variants 
of such networks are created by adding or expanding layers within 
individual blocks instead of growing them from one end. For instance, 
VGG-C (with 16 convolutional layers) is obtained by adding one layer 
to each of the last three blocks of VGG-B (with 13 convolutional 
layers) \cite{Simonyan2014}. 
%

To construct the MotherNet for every block, we select as many 
convolutional layers to include in the MotherNet as the 
network in $E$ with the least number of layers in that block. Every 
layer within a block is constructed such that it has the least number 
of filters and the smallest filter size of any layer at the same 
position within that block.
%
Figure \ref{fig:example_block_by_block} shows this approach applied 
to an ensemble of convolutional networks with three blocks each. 
The resulting MotherNet is shown at the bottom in bold. In this 
Figure, unshaded rectangles represent convolutional layers. 
To denote the structural hyperparameters of a convolutional 
layer we use the following notation: 
\texttt{<filter\_size>:<filter\_number>}. 



%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
\subsection{Training} 

We describe how MotherNets train an ensemble. 


\boldPara{Training the MotherNet.} 
First, the MotherNet is trained from scratch using the entire 
data set until convergence. The MotherNet learns a good core 
representation of the data as well as captures relevant 
relations between the input features and the output labels. 

%This phase reduces bias as the MotherNet 
%learns a good core representation of the data

\boldPara{Hatching ensemble networks.} Once the MotherNet 
is trained, the next step is to generate every ensemble 
network by expanding the MotherNet through a sequence 
of function-preserving transformations. We call this 
process hatching. Hatching yields the ensemble networks 
with possibly larger size (more parameters) than the 
MotherNet but representing the same function as learnt 
by the MotherNet. 
%
The hatching process is instantaneous as generating 
every ensemble network requires a single pass on the 
MotherNet. 
%Now, every 
%hatched ensemble network with size (number of parameters) 
%larger than the MotherNet now has some new untrained parameters 
%that we further train.  

%\todo{How does network morphism apply these transformations?}
%
%\todo{Is there something interesting about hatching that we 
%should specifically mention in the paper?}

\boldPara{Training ensemble networks.} 
The hatched ensemble networks are trained using bootstrap 
aggregation (bagging) \cite{Breiman1996}: 
%
Every hatched network is trained using a separate bagged 
set $B$. $B$ is the same size as the original data set but 
it is created from the original data set through sampling 
with replacement. 
%
Bagging is an effective and widely used method to create diversity 
and to reduce the variance of ensembles 
\cite{Guzman2014,Hansen1990,Stefan2015}. This is because different 
models in the ensemble are trained using different overlapping 
subsets of the data. 
%
However, previous work has shown that training neural network 
ensembles through bagging results in decreased generalization 
accuracy as it reduces the number of unique data items seen by 
individual neural networks. Since, neural networks have a large 
number of parameters they are affected relatively more from this 
reduction in unique data items than ensembles of other classifiers 
such as decision trees or SVMs \cite{Domingos1999,Lee2015}. 
%
Hatching the networks from the MotherNet and then further training 
them using bagging overcomes this problem. We observe that by 
training the hatched networks through bagging, we converge faster 
as well as achieve generalization accuracy that is comparable to 
training using the entire data set. 


\boldPara{Parallel training and optimizations.} The training process described 
above can be easily parallelized. Every MotherNet can be trained 
independently and in parallel. Similarly, when ensemble networks 
are hatched from the MotherNet, they can also be trained separately 
and in parallel. Standard approaches to parallelize the training 
of these individual network are all applicable \cite{Dean2012}. 
%
In addition, existing approaches to accelerate the training of individual 
neural networks as well as improve their generalization accuracy can 
all be incorporated into our training phases 
\cite{Huang2016,Huang2017,Ioffe2015,Singh2016,Srivastava2014,Wan2013}.

%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%  
\subsection{Controlling difference between the MotherNet 
and ensemble networks} 

%%% %%% %%%%
\begin{figure}[t]
		\centering
		\includegraphics[width=\linewidth]{images/schematic/example_block_by_block}
		\caption{\label{fig:example_block_by_block} Constructing the MotherNet 
		block-by-block for ConvNets.}
\end{figure}

\begin{algorithm}
	\caption{Cluster ensemble networks}\label{alg:cluster_ens}
			%
	\textbf{Input:} E: ensemble networks sorted by size; 
	$\tau$: clustering parameter;
	%
	\BlankLine
	\textbf{Initialize:} start $\gets0$; clusterID $\gets 0$; 
	\BlankLine
	\While{all net. in E are not assigned to a cluster}{
		cluster = [];\\
		\For{$i \gets$ start \ldots len(E)}{
			cluster.append(E[i]);\\
		\If{not satisfyClusteringCondition(cluster, $\tau$)}
			{
			start $\gets i$;\\ 
			clusterID++;\\ 
			break;
			}
			E[i].cluster = clusterID;
		}
	}
\end{algorithm}

%%% %%% %%% 

The size of the MotherNet is limited by the size of the 
smallest network in the ensemble. 
%
For ensembles that have a large difference in size between 
the smallest and the largest networks, there will be a 
correspondingly large size difference between at least one 
ensemble network and the MotherNet. This may lead to a 
scenario where the MotherNet is much smaller than some of 
the networks and can only capture an insignificant amount 
of structural commonality. 
%
To avoid such cases, we divide the ensemble networks $E$ into 
clusters and construct a separate MotherNet for every cluster. 
%
In forming these clusters, we ensure that for every ensemble 
network, at least a fraction $\tau$ of its parameters originate 
from its MotherNet. 
%
Formally, we divide $E$ into $G$ clusters 
$\{C_0, C_1, \dots C_{G-1}\}$. 
%
Every cluster satisfies the following condition: Let $M_g$ be 
the MotherNet for the cluster $C_g$ with networks 
$\{C_g^j\}$, then: $\forall  C_g^j \in C_g: {|C_g^j| - |M_g|} < \tau	 \cdot {|C_g^j|}$, 
%
where $|C_g^j|$ and $|M_g|$ is the size (in terms of number of 
parameters) of $C_g^j$ and $M_g$ respectively.
%

The clustering parameter $\tau$ controls the tradeoff 
between the number of new parameters (or weights) introduced 
when hatching ensemble networks and the total number of 
clusters. 
%
For instance, on one extreme, if $\tau$ is set to $1$, then 
we will have as many clusters as the size of $E$ i.e., every 
network will be its own MotherNet. On the other extreme, if 
$\tau$ is set close to $0$, we will end up with one cluster 
and the MotherNet can be arbitrarily small. 
%In our experiments, we set the value of $\tau$ to $0.5$. This 
%ensures that a majority of the parameters in every ensemble 
%originates from its MotherNet.

\boldPara{Clustering algorithm.} 
For a given $\tau$, we provide an algorithm to create the 
minimum amount of clusters, while satisfying the clustering 
condition. 
%
A naive strategy to achieve this is to look at all possible 
ways of partitioning $E$ (exponentially many), filter those 
that satisfy the clustering condition, and pick the 
partitioning with the least number of clusters. 
%
However, we observe that we can reduce this exponential time 
complexity to linearithmic ($n \log n$) time by first ordering 
the networks with respect to the network size (number of 
parameters). 



This is driven by the following observation: Given a cluster 
that satisfies the clustering condition with the size of 
the smallest and the largest network being $C_-$ and $C_+$ 
respectively, then, all networks that have size in $\{|C_-|,|C_+|\}$ 
can be added to this cluster without violating the clustering 
condition. However, networks with size outside $\{|C_-|,|C_+|\}$, 
if added to this cluster may cause the cluster to violate the 
clustering condition. 
%
These networks should be considered in the order of their size, 
when expanding the cluster. This is because if networks 
$X: |X| > |C_+|$ and $Y: |Y| < |C_-|$ cannot be added to the 
cluster, then no element $X_+$ larger than $X$ or $Y_-$ 
smaller than $Y$ can be added to the cluster either.
%
Consequently, when we order the networks in $E$ by size, we 
only need to look at consecutive sequences of the networks and 
not all possible partitionings of $E$.

%

Algorithm \ref{alg:cluster_ens} describes our strategy 
to construct clusters. 
%
As an input it receives $E$ with networks sorted in the 
ascending order of the number of parameters. 
%
The algorithm starts with an empty cluster. It adds networks 
from $E$ into the cluster one-by-one in order until the cluster 
no longer satisfies the clustering condition. 
At this point, the last network that was added to the cluster is 
removed, a new cluster is initialized and the process is repeated 
(i.e., remaining unassigned elements from $E$ are added into the 
next cluster). 

==> files/main_may_1.tex <==
\section{MotherNet}

We describe how to construct a MotherNet and explain how it can be 
used to quickly train an ensemble of neural networks. 


\boldPara{MotherNet.} 
% Definition: 
Given an ensemble with different neural network architectures, we 
define the MotherNet as \textit{any neural network architecture 
from which members of the given ensemble can be obtained by 
applying a sequence of function-preserving transformations}. 
% MotherNetMax: 
Given an ensemble, there could be many such MotherNets as many 
architectures with parameters less than all members of the ensemble 
can be expanded through function-preserving transformations to generate 
the ensemble and can thereby function as a MotherNet. 
However, the size of one of them will dominate the size of all other 
MotherNets. We call this architecture the MotherNetMax and it captures 
the largest structural commonality that exists between all the networks 
in the ensemble. 
%

Here we provide a method to construct the MotherNetMax. In scenarios 
with resource constraints such as available memory and compute power, 
one may consider constructing a smaller MotherNet with number of 
parameters that satisfy resource constraints.


\subsection{Constructing the MotherNet} 
Given 
$E = \{N_0, N_1, \dots N_{K-1}\}$, an ensemble of $K$ neural 
network models (where $N_k$ denotes a neural network model in 
the ensemble). We explain how to construct the MotherNetMax 
$M$ for ensembles of both fully-connected and convolutional 
neural networks. 

%% Fully-connected Networks
\textbf{Fully-connected networks.} 
For ensembles of fully-connected networks, $M$ is constructed 
as follows: First, its input and output layers have the same 
structure as all the networks in $E$, since they are all trained 
for the same task. Then, $M$ is initialized with as many hidden 
layers as the shallowest network in $E$.  
% 
Then, we construct the hidden layers of $M$ one-by-one going from 
the input to the output layer such that the structure of the $i$-th 
hidden layer of $M$ is the same as the $i$-th hidden layer from the 
networks in $E$ with the least number of parameters. 

For instance, consider the example in Figure \ref{fig:example}a, 
given an ensemble with two three-layered networks and one four-layered 
network, the mother network is constructed with just three layers. 
Furthermore, every layer of the MotherNet is constructed such that it 
has the same structure as the layer with the least number of parameters 
at that position (shown in bold in Figure \ref{fig:example}a). 

%% ConvNets
% ConvNets follow a set structure.
%In the case of convolutional neural networks, we construct the 
%MotherNetMax $M$ as follows: 
%

\textbf{Convolutional neural networks.} 
%For convolutional neural networks, we follow the same strategy i.e., 
%we construct the MotherNetMax layer-by-layer. However, layers in 
%convolutional neural networks are characterized by both the number 
%of filters (or convolutional channels) and the filter size. Every 
%convolutional layer in the MotherNetMax has as many filters as the 
%layer at that position with the least number of filters. The filter 
%size of that layer is set to be the smallest at that layer. Again, 
%this ensures that we can instantiate every member of the ensemble 
%by applying a sequence of function-preserving transformations. 
%%
%We discuss specific types of convolutional neural networks and 
%how we construct MotherNetMax for them: 
%
Convolutional neural network architectures consist of blocks of 
convolutional layers separated by max-pooling layers 
\cite{He2016,Shazeer2017,Simonyan2014,Szegedy2015}. For instance, 
VGGNets are composed of five blocks of convolutional layers 
separated by max-pooling layers, whereas, DenseNets consist of 
four blocks of densely connected convolutional layers. 
These blocks are then followed by one or more fully-connected 
layers. 
%
For these networks, we construct the MotherNetMax $M$ 
block-by-block instead of layer-by-layer. 
The intuition behind this approach is that deeper or wider variants 
of such networks are created by adding or expanding layers within 
individual blocks instead of growing them from one end. For example, 
VGG-C (with 16 convolutional layers) is obtained by adding one layer 
to each of the last three blocks of VGG-B (with 13 convolutional layers). 
%

To construct the MotherNet block-by-block for every block, we select 
as many convolutional layers to include in the MotherNetMax as the 
network in $E$ with the least number of layers in that block. Every 
layer within a block is constructed such that it has the least number 
of filters and the smallest filter size for any layer at the same 
position within that block.


%\textbf{Inception Networks.} For the inception network, we can 
%basically apply the same approach, for every layer, we keep the 
%least number of parameters. 

\todo{Revise the example figure.}

\todo{Why is this a good way to construct the MotherNet?}

\todo{What if this results in a really bad architecture for 
training?}

\todo{Maybe a figure and example here can really be helpful.}

% 

\subsection{Training}

\cmt{Pending.}

%\cmt{Given this formulation, there are a few options to train:
%\begin{enumerate}
%	\item Train $M$ to convergence $\rightarrow$ train $E$.
%	\item Co-train $M$ and $E$.
%	\item Train $M$ until a specified accuracy $\rightarrow$ 
%	co-train $M$ and $E$ until it makes no sense to co-train 
%	$M$ $\rightarrow$ train only $E$.
%\end{enumerate}}
%
%\cmt{We can use approaches the leverage knowledge across different 
%networks in $E$ while they are being trained. For instance, we 
%can use the mimicry loss from Deep Mutual Learning as well as 
%the diversity inducing loss from ``Why M Heads are Better than 
%One?''. My intuition is that using such losses does not scale well 
%as far as training is concerned. Training $E$ with bagging is on 
%the other hand embarrassingly parallel. To perform an update in 
%every epoch for this method, one needs to look at the output 
%produced by all the networks in the cohort i.e., one needs to 
%wait for all the networks to finish processing a mini-batch 
%before an update. Furthermore, we can say that bagging produces 
%sufficient diversity and the MotherNet produces good core similarity 
%between the networks.}
%
%Once the MotherNet is constructed, the training proceeds in three 
%phases: 
%%
%We begin by only training the MotherNet, then we transition to 
%co-train both the MotherNet and the ensemble networks, and finally 
%we train just the ensemble networks. Figure \ref{fig:example_phase_diag}b 
%depicts the three-phased training process. We discuss each of the phases 
%in detail: 
%
%\todo{We need to add reasoning for why we train the network in 
%this particular way.}
%
%%During the first phase, only the MotherNet is trained until it 
%%reaches a specified accuracy.
%%%
%%Then, by using function-preserving transformations, networks in 
%%the ensemble E are instantiated from the MotherNet. During the 
%%second phase, both the MotherNet and the individual networks are 
%%trained. We monitor the accuracy gained per FLOP for the MotherNet 
%%and the ensemble networks during this phase. 
%%%
%%Whenever the gain is higher for the ensemble network, we transition 
%%into the third phase, where we just train the ensemble networks. 
%
%\boldPara{Phase 1.} The training process begins with only the MotherNet, 
%which is trained from scratch using the entire training data set (i.e., 
%no bagging). When the MotherNet reaches a pre-specified accuracy, we 
%apply functional preserving transformations (Net2WiderNet and 
%Net2DeeperNet) to instantiate each of the networks in the ensemble 
%$E$. This allows us to create ensemble networks with the same function 
%(and accuracy) as the MotherNet but with structures that are 
%representationally richer i.e., have more parameters. Now, we 
%transition to the second phase. 
%
%\boldPara{Phase 2.}  In this phase, we co-train the MotherNet with 
%the ensemble networks. We use the whole data set to train the MotherNet 
%and use bagging to train the ensemble networks as bagging is a typical 
%and efficient method to train ensembles \cite{Dietterich2000}. During 
%this phase, we monitor the accuracy of the MotherNet and the combined 
%accuracy of the ensemble networks after every training epoch. If the 
%MotherNet results in higher accuracy, we use it to re-instantiate 
%ensemble networks through function-preserving transformations and 
%then repeat this process. If the combined accuracy of the ensemble 
%networks is higher, then we transition to the third phase.  
%%
%
%\boldPara{Phase 3.} In this phase, only the ensemble networks are trained to
%convergence. 

==> files/main_may_14.tex <==
\section{Training Ensembles through MotherNets}

% Overview
%MotherNet accelerates the training of explicit ensembles of neural 
%networks by capturing the structural similarity that exists between 
%different networks in the ensemble. The MotherNet is then trained 
%using the entire data set. Once trained, the learnt function is 
%transferred to the ensemble networks. These ensemble networks are 
%then trained using bootstrap aggregation and converge much faster 
%than training from scratch. This process is depicted in Figure 
%\ref{fig:example}. 
%
%Overall, this results in significant decrease in training time 
%as compared to existing approaches, while achieving comparable 
%ensemble accuracy. Further, as the size of the ensemble increases, 
%the improvement in training time also increases as every additional 
%network can be hatched from the MotherNet and then quickly trained 
%to convergence. In this way, MotherNet makes it feasible to 
%effectively train large ensembles of deep neural networks.
%
First, we define the MotherNet and then, explain how we use it 
to train an ensemble of neural networks. 

\boldPara{MotherNet.} 
Given an ensemble with different neural network architectures, the 
MotherNet captures the largest structural similarity 
between them. Formally, it is the largest neural network from which 
members of an ensemble can be obtained by applying a sequence of 
function-preserving transformations. Function-preserving 
transformations allow us to expand the size of a trained network, 
while preserving its function \cite{Chen2015,Wei2016,Wei2017}. 
Given an ensemble, many neural networks with size less than all 
of the ensemble networks can be expanded through function-preserving 
transformations to obtain the ensemble networks. 
The MotherNet is defined to be the largest of such networks. It 
follows from this definition that: 
(i) ensemble networks hatched from the MotherNet can immediately 
inherit its function (mapping between input data items and output 
labels) and 
(ii) the structure of the MotherNet is smaller than or equal to the 
ensemble network with the smallest size. 


\boldPara{Function-preserving transformations.} 
%Given a neural network with a certain function (mapping between 
%input data items and output labels), function-preserving 
%transformations can be applied to create another neural network 
%with more model capacity (parameters) while preserving the original 
%function \cite{Chen2015,Wei2016,Wei2017}. 
%
We provide a brief overview of function-preserving transformations. 
They allow us to grow the size of a neural network, while ensuring 
that the function is preserved. 
%
Function-preserving transformations enable the 
ensemble networks to \textit{inherit} the learnt function from 
the MotherNet. 
%This provides a good starting point for further 
%training resulting in higher generalization accuracy as well 
%as faster convergence of the ensemble networks. 
%
%
We use three classes of function-preserving transformations 
as shown in Figure \ref{fig:FPT} and they allow us to increase the 
depth of the network (Figure \ref{fig:FPT}a), widen the network 
layers (Figure \ref{fig:FPT}b), and grow the size of convolutional 
filters (Figure \ref{fig:FPT}c). 
% 
There are two distinct approaches to achieve these transformations: 
Net2Net and Network Morphism. 
%
Net2Net increases the capacity of the given network by adding identity 
layers or by replicating existing weights \cite{Chen2015}. 
%
Network Morphism, on the other hand, derives sufficient and necessary 
conditions that when satisfied will extend the network while preserving 
its function and provides algorithms to solve for those conditions 
\cite{Wei2016,Wei2017}. 
%
In MotherNet, we adopt the second approach 
\footnote{There is ongoing research on function-preserving 
transformations. Novel and better approaches introduced in 
the future can also be applied within the context of the 
MotherNet.} 
i.e., Network Morphism, as 
it has been shown to serve as a better starting point for further 
training as compared to Net2Net \cite{Wei2016,Wei2017}. \rev{These 
transformations work for a wide range of neural networks including 
VGGNets and ResNets \cite{Wei2016,Wei2017}.}
%

\cmt{Based on space, we may add another paragraph about FPTs here.}

\begin{figure}[t!]
	\includegraphics[width=\linewidth]{images/schematic/example}
	\caption{\label{fig:example} MotherNet accelerates the training 
	of neural network ensembles.}
\end{figure}

\begin{figure}[]
	\includegraphics[width=\linewidth]{images/schematic/FPT}
	\caption{\label{fig:FPT} MotherNet uses three function-preserving 
	transformations to hatch ensemble networks.}
	\vspace{-0.175in}
\end{figure}


% MotherNetMax: 
%\boldPara{MotherNet.}
%The architecture of the MotherNet is strictly smaller (have less 
%depth and layer-wise width) than all of the ensemble networks. 
%This is because we should be able to expand the MotherNet to 
%generate all the ensemble networks through function-preserving 
%transformations. 
%%
%Given an ensemble, there could be many MotherNets as many architectures 
%with parameters less than all members of the ensemble can be expanded 
%through function-preserving transformations to generate the ensemble. 
%However, the size of one of them will dominate the size of all other 
%MotherNets. We call this network the MotherNetMax and it captures 
%the largest structural commonality that exists between all the networks 
%in the ensemble. 


%
\subsection{Constructing the MotherNet}

First, we provide a method to construct the MotherNet $M$ from 
an ensemble $E = \{N_0, N_1, \dots N_{K-1}\}$ of $K$ neural 
networks (where $N_k$ denotes a neural network architecture 
in the ensemble). 
%
We describe how to construct $M$ for ensembles of both 
fully-connected and convolutional neural networks. 
%
Then, we explain how we handle the case 
where networks in the ensemble have a large difference in size. 

%In scenarios 
%with resource constraints such as available memory and compute power, 
%we can construct a smaller MotherNet by pruning the MotherNetMax.
%
%
%Let $E = \{N_0, N_1, \dots N_{K-1}\}$ be an ensemble of $K$ 
%neural network architectures (where $N_k$ denotes a neural 
%network architectures in the ensemble). We explain how to 
%construct the MotherNet $M$ for ensembles of both 
%fully-connected and convolutional neural networks. 

%% Fully-connected Networks
\textbf{Fully-connected networks.} 
For ensembles of fully-connected neural networks, $M$ is 
constructed as follows: First, its input and output layers 
have the same structure as all the networks in $E$, since 
they are all trained for the same task. Then, $M$ is 
initialized with as many hidden layers as the shallowest 
network in $E$.  
% 
Then, we construct the hidden layers of $M$ one-by-one going from 
the input to the output layer such that the structure of the $i$-th 
hidden layer of $M$ is the same as the $i$-th hidden layer of the 
network in $E$ with the least number of parameters. 


Figure \ref{fig:example}a depicts an example of an ensemble, 
with two three-layered networks and one four-layered network, 
where the MotherNet consists of three layers. 
%
Every layer of the MotherNet is constructed such that it 
has the same structure as the layer with the least number of parameters 
at that position (shown in bold in Figure \ref{fig:example}a). 

%% ConvNets
% ConvNets follow a set structure.
%In the case of convolutional neural networks, we construct the 
%MotherNetMax $M$ as follows: 
%
%%% %%% %%%
%\begin{wrapfigure}{R}{0.5\textwidth}
%\begin{algorithm}[H]
%\caption{Cluster ensemble networks}\label{alg:cluster_ens}
%%
%\textbf{Input:} E: ensemble networks sorted by number of parameters\;
%%
%\BlankLine
%\textbf{Initialize:} start $\gets0$; clusterID $\gets 0$\; 
%\While{all net. in E are not assigned to a cluster}{
%	cluster = []\;
%	\For{$i \gets$ start \ldots len(E)}{
%		cluster.append(E[i])\;
%	\If{not goodCluster(cluster)}
%		{
%			start $\gets i$; clusterID++; break;
%		}
%	E[i].cluster = clusterID;
%	}
%}
%\end{algorithm}
%\end{wrapfigure}
%%% %%% %%% 

\textbf{Convolutional neural networks.}  
%
Convolutional neural network architectures consist of blocks of 
convolutional layers separated by max-pooling layers 
\cite{He2016,Shazeer2017,Simonyan2014,Szegedy2015}. 
These blocks are then followed by another block of one or more 
fully-connected layers.
For instance, VGGNets are composed of five blocks of convolutional 
layers separated by max-pooling layers, whereas, DenseNets consist 
of four blocks of densely connected convolutional layers. 
%
For such networks, we construct the MotherNet $M$ 
block-by-block instead of layer-by-layer. 
The intuition is that deeper or wider variants 
of such networks are created by adding or expanding layers within 
individual blocks instead of growing them from one end. For instance, 
VGG-C (with 16 convolutional layers) is obtained by adding one layer 
to each of the last three blocks of VGG-B (with 13 convolutional 
layers) \cite{Simonyan2014}. 
%

To construct the MotherNet for every block, we select as many 
convolutional layers to include in the MotherNet as the 
network in $E$ with the least number of layers in that block. Every 
layer within a block is constructed such that it has the least number 
of filters and the smallest filter size of any layer at the same 
position within that block.
%
Figure \ref{fig:example_block_by_block} shows this approach applied 
to an ensemble of convolutional networks with three blocks each. 
The resulting MotherNet is shown at the bottom in bold. In this 
Figure, unshaded rectangles represent convolutional layers. 
To denote the structural hyperparameters of a convolutional 
layer we use the following notation: 
\texttt{<filter\_size>:<filter\_number>}. 

%%% %%% %%%%
\begin{figure}[t]
	\begin{minipage}{0.35\textwidth}
		\includegraphics[width=\linewidth]{images/schematic/example_block_by_block}
		\caption{\label{fig:example_block_by_block} Constructing MotherNet 
		block-by-block}
	\end{minipage}
	\hspace{0.025\textwidth}
	\begin{minipage}{0.6\textwidth}
		
		\begin{algorithm}[H]
			\caption{Cluster ensemble networks}\label{alg:cluster_ens}
			%
			\textbf{Input:} E: ensemble networks sorted by size\;
			\hspace{0.425in}$\tau$: clustering parameter\;
			%
			\BlankLine
			\textbf{Initialize:} start $\gets0$; clusterID $\gets 0$\; 
			\BlankLine
			\While{all net. in E are not assigned to a cluster}{
			cluster = []\;
			\For{$i \gets$ start \ldots len(E)}{
				cluster.append(E[i])\;
			\If{not satisfyClusteringCondition(cluster, $\tau$)}
				{
				start $\gets i$\; clusterID++\; 
				break;
				}
			E[i].cluster = clusterID;
				}
			}
\end{algorithm}

	\end{minipage}
	\vspace{-0.2in}
\end{figure}
%%% %%% %%% 

\cmt{Maybe we are spending too much real-estate on clustering}

\todo{Consider reversing the order. Say that we are introducing 
a way to control how far the MN fall from the EN. This can be 
used in a few scenarios ...}

\boldPara{Clustering ensemble networks.} 
To handle scenarios, where ensemble networks in $E$ have large 
differences in their size (number of parameters), we divide $E$ 
into clusters; for every cluster we construct a separate MotherNet. 
In forming these clusters, we ensure that for every ensemble 
network, at least a fraction $\tau$ of its parameters originate 
from its MotherNet. 
%
Formally, we divide the ensemble networks $E$ into $G$ clusters 
$\{C_0, C_1, \dots C_{G-1}\}$. 
%
Every cluster satisfies the following property: Let $M_g$ be 
the MotherNet for the cluster $C_g$ with networks 
$\{C_g^j\}$, then: 

\begin{equation}
	\forall  C_g^j \in C_g: {|C_g^j| - |M_g|} < \tau	 \cdot {|C_g^j|}
	\label{eq:clustering_condition}
\end{equation}
\vspace{-0.1in}

%
where $|C_g^j|$ and $|M_g|$ is the size (in terms of number of 
parameters) of $C_g^j$ and $M_g$ respectively.
%

The clustering parameter $\tau$ controls the tradeoff 
between the number of new parameters (or weights) introduced 
when hatching ensemble networks and the total number of 
clusters. 
%
For instance, on one extreme, if $\tau$ is set to $1$, then 
we will have as many clusters as the size of $E$ i.e., every 
network will be its own MotherNet. On the other extreme, if 
$\tau$ is set close to zero, we will end up with one cluster 
and the MotherNet can be arbitrarily small. 
In our experiments, we set the value of $\tau$ to $0.5$. This 
ensures that a majority of the parameters in every ensemble 
originates from its MotherNet.

For a given $\tau$, we provide an algorithm to create the 
minimum amount of clusters, while satisfying the condition 
from Equation \ref{eq:clustering_condition}. 
%
A naive strategy to achieve this is to look at all possible 
ways of partitioning $E$ (exponentially many), filter those 
that satisfy the condition from Equation 
\ref{eq:clustering_condition}, and pick the partitioning 
with the least number of clusters. 
%
However, we observe that we can reduce this exponential time 
complexity to linearithmic ($n \log n$) time by first ordering 
the networks with respect to the network size (number of 
parameters). 

\todo{Verify the following statement.}

This is driven by the observation that given a cluster 
that satisfies the clustering condition (Equation 
\ref{eq:clustering_condition}) with the size of the smallest 
and the largest network being $C_-$ and $C_+$ respectively. 
Then all networks that have size in $\{|C_-|,|C_+|\}$ can be 
added to this cluster without violating the clustering condition. 
However, networks with size outside $\{|C_-|,|C_+|\}$, if added 
to this cluster may cause the cluster to violate the clustering 
condition. 
%
These networks should be considered in the order of their size, 
when expanding the cluster. This is because if networks 
$X: |X| > |C_+|$ and $Y: |Y| < |C_-|$ cannot be added to the 
cluster, then no element $X_+$ larger than $X$ or $Y_-$ 
smaller than $Y$ can be added to the cluster either.
%
Consequently, when we order the networks in $E$ by size, we 
only need to look at consecutive sequences of the networks and 
not all possible partitions of $E$.

%

Algorithm \ref{alg:cluster_ens} describes our strategy 
to construct clusters. 
%
As an input it receives $E$ with networks sorted in the 
ascending order of the number of parameters. 
%
The algorithm starts with an empty cluster. It adds networks 
from $E$ into the cluster one-by-one in order until the cluster 
no longer satisfies the clustering condition. 
At this point, the last network that was added to the cluster is 
removed, a new cluster is initialized and the process is repeated 
(i.e., remaining unassigned elements from $E$ are added into the 
next cluster). 

\todo{This algorithm works, but is it an overkill? Do we need 
to build the MotherNets to make the decisions?}

\todo{How do we prove that this does result in the least 
number of clusters?}

\todo{Does this also minimize the overall difference 
between MN and the individual ensembles?}
%\boldPara{Clustering ensemble networks.} 
%In scenarios where $E$ has networks with a large difference in 
%network size (number of parameters), we divide the networks in 
%$E$ into clusters.  We construct and train a separate MotherNet 
%for every cluster. In forming these clusters, we ensure that for 
%every network, a majority of its parameters originate from its 
%MotherNetMax when it is hatched. 
%
%Formally, we divide the ensemble networks $E$ into $G$ clusters 
%$\{C_0, C_1, \dots C_{G-1}\}$. For every cluster, we construct 
%a separate MotherNetMax. 
%%
%Every cluster satisfies the following property: Let $M_g$ be 
%the MotherNetMax for the cluster $C_g$ with networks 
%$\{C_g^j\}$, then: 
%
%\begin{equation}
%	\forall  C_g^j \in C_g: |C_g^j| - |M_g| < |M_g|	
%	\label{eq:clustering_condition}
%\end{equation}
%
%
%
%where $|C_g^j|$ and $|M_g|$ is the size (number of 
%parameters) of $C_g^j$ and $M_g$ respectively. This condition 
%ensures that more than half of the parameters come directly 
%from the MotherNet and are not introduced through 
%function-preserving transformations. \rev{Our experiments suggest 
%that this is a reasonable condition to impose.}
%%
%
%\todo{Why do we do this? Can we do experiments to show that this 
%is reasonable?}
%
%
%Algorithm \ref{alg:cluster_ens} provides a strategy to construct 
%clusters while satisfying the condition from Equation 
%\ref{eq:clustering_condition}. 
%%
%As an input it receives $E$ with networks sorted in the ascending 
%order of the number of parameters. 
%%
%The algorithm starts with an empty cluster. It adds networks 
%from $E$ into the cluster one-by-one in order until the cluster 
%no longer satisfies the condition in Equation \ref{alg:cluster_ens}. 
%At that point, the last network that was added to the cluster is 
%removed, a new cluster is initialized and the process is repeated 
%(i.e., remaining unassigned elements from $E$ are added into the 
%next cluster). 
%
%\rev{The conjecture is that this does the clustering in a way that 
%least number of clusters are created \ref{eq:clustering_condition}.} 
%
%
%
%%
%\todo{What exactly is it that this algorithm is trying to optimize for? 
%the size? the difference? the number of MotherNets to train?}
%
%\todo{Would there be any difference if we try to build these groups 
%in the descending or the ascending order?} 
%I think the boundaries will 
%still be the same. 

\subsection{Training} 

\boldPara{Training MotherNet.} 
The MotherNet is trained from scratch using the entire data set 
until convergence. The MotherNet learns a good core representation 
of the data as well as captures relevant relations between the 
input features and the output labels. 

%This phase reduces bias as the MotherNet 
%learns a good core representation of the data

\boldPara{Hatching ensemble networks.} Once the MotherNet is 
trained, the next step is to generate every ensemble network 
by expanding the MotherNet through a sequence of 
function-preserving transformations. We call this process 
hatching. Hatching yields all the ensemble networks with possibly 
different architectures but representing the same function as 
learnt by the MotherNet. 

\todo{How does network morphism apply these transformations?}

\todo{Is there something interesting about hatching that we 
should specifically mention in the paper?}

%In applying these function-preserving 
%transformations, we ensure that the relative position of the 
%layers from the MotherNet is also preserved in every ensemble 
%network. This is inline with the observation that layers in 
%neural networks progressively learn more complicated and 
%specific representations of the data and as such the order of 
%the layers is consequential \cite{Yosinski2014}.


\boldPara{Training ensemble networks.} 
The hatched ensemble networks are trained using sub-sampling 
from the data set i.e., bootstrap aggregation (bagging). We 
train every hatched network using a separate bagged set $B$. 
$B$ is the same size as the original data set but it is 
created from the original data set by sampling with 
replacement. 
%
Bagging is an effective method to create diversity and reduce 
variance of an ensemble \cite{Guzman2014,Hansen1990,Lee2015}. 
This is because different models in the ensemble are trained 
using different overlapping subsets of the data. 
%
However, bagging has been shown to not perform as well 
for neural network ensembles as it reduces the number of 
unique data items seen by individual neural networks. This 
is because neural networks have a relatively large number 
of parameters and suffer from reduction in unique data items 
\cite{Domingos1999,Lee2015}. Hatching the networks from a 
well-trained MotherNet and then training them using bagging 
overcomes this problem. We observe that by training the hatched 
networks through bagging, we converge faster and achieve 
generalization accuracy comparable to training the hatched 
networks through the entire data set. 


%. The training proceeds in two phases: 
%% Phase 1
%In the first phase, all MotherNets are trained from scratch 
%using the entire data set until they converge. This phase 
%reduces bias as the MotherNets are trained on the entire 
%data set to convergence and their parameters learn a good 
%core representation of the data. 
%%
%This representation is then immediately transferred to 
%the ensemble networks in a process we call \textit{hatching}. 
%% Phase 2
%Then, in the second phase, the hatched ensemble networks are 
%trained using sub-sampling from the data set i.e., bootstrap 
%aggregation. This phase explicitly creates diversity within 
%the ensemble networks that reduces variance and improves 
%the generalization accuracy of an ensemble classifier 
%\cite{Guzman2014,Hansen1990,Lee2015}.

\boldPara{Parallel training.} Each of these phases can be easily 
parallelized: Every MotherNet can be trained in parallel. Similarly, 
when ensemble networks are hatched from the MotherNet, they can also 
be trained in parallel. Training of an individual network can also 
be parallelized using standard approaches \cite{Dean2012}. 
%
Further, existing approaches to accelerate the training of individual 
neural networks as well as improve their generalization accuracy can 
all be incorporated into our training phases 
\cite{Huang2016,Huang2017,Ioffe2015,Singh2016,Srivastava2014,Wan2013}.

%
%as follows: The MotherNet corresponding 
%to every cluster is trained to convergence on the entire data 
%set. Then, the ensemble networks corresponding to that cluster 
%are hatched from the MotherNet through a sequence of 
%function-preserving transformations. At this point, every member 
%of the ensemble has exactly the same function as the MotherNet, 
%but with additional parameters that can be further trained. 
%%
%At this point, the bias associated with every network is quite 
%low. This is so because we observe that compared to the approach 
%where we train each of the networks from scratch using bagging, 
%the ensemble accuracy is already much higher. 

%\rev{
%\begin{itemize}
%	\item Training data -- full vs. bagging. 
%	\item How much to train -- convergence vs. fixed number of epochs.
%	\item Learning hyperparameters. 
%\end{itemize}
%}

%\todo{Is the per epoch training time the same for bagging and 
%full-data set?}
%
%\todo{Does it not always make sense to use full data set to 
%train the ensemble networks?}
%
%\todo{In all approaches of bagging, do we always subsample 
%the data set to have the same size?}


%\cmt{Explain how existing approaches have used exclusively full-training 
%the neural network ensembles because bagging does not work as there is 
%not enough data to train networks with large parameters. However, with 
%our approach, we show that bagging can still be used as a viable method 
%to train the ensemble networks, once they have been hatched from the 
%MotherNet.}



%\cmt{Given this formulation, there are a few options to train:
%\begin{enumerate}
%	\item Train $M$ to convergence $\rightarrow$ train $E$.
%	\item Co-train $M$ and $E$.
%	\item Train $M$ until a specified accuracy $\rightarrow$ 
%	co-train $M$ and $E$ until it makes no sense to co-train 
%	$M$ $\rightarrow$ train only $E$.
%\end{enumerate}}
%
%\cmt{We can use approaches the leverage knowledge across different 
%networks in $E$ while they are being trained. For instance, we 
%can use the mimicry loss from Deep Mutual Learning as well as 
%the diversity inducing loss from ``Why M Heads are Better than 
%One?''. My intuition is that using such losses does not scale well 
%as far as training is concerned. Training $E$ with bagging is on 
%the other hand embarrassingly parallel. To perform an update in 
%every epoch for this method, one needs to look at the output 
%produced by all the networks in the cohort i.e., one needs to 
%wait for all the networks to finish processing a mini-batch 
%before an update. Furthermore, we can say that bagging produces 
%sufficient diversity and the MotherNet produces good core similarity 
%between the networks.}
%
%Once the MotherNet is constructed, the training proceeds in three 
%phases: 
%%
%We begin by only training the MotherNet, then we transition to 
%co-train both the MotherNet and the ensemble networks, and finally 
%we train just the ensemble networks. Figure \ref{fig:example_phase_diag}b 
%depicts the three-phased training process. We discuss each of the phases 
%in detail: 
%
%\todo{We need to add reasoning for why we train the network in 
%this particular way.}
%
%%During the first phase, only the MotherNet is trained until it 
%%reaches a specified accuracy.
%%%
%%Then, by using function-preserving transformations, networks in 
%%the ensemble E are instantiated from the MotherNet. During the 
%%second phase, both the MotherNet and the individual networks are 
%%trained. We monitor the accuracy gained per FLOP for the MotherNet 
%%and the ensemble networks during this phase. 
%%%
%%Whenever the gain is higher for the ensemble network, we transition 
%%into the third phase, where we just train the ensemble networks. 
%
%\boldPara{Phase 1.} The training process begins with only the MotherNet, 
%which is trained from scratch using the entire training data set (i.e., 
%no bagging). When the MotherNet reaches a pre-specified accuracy, we 
%apply functional preserving transformations (Net2WiderNet and 
%Net2DeeperNet) to instantiate each of the networks in the ensemble 
%$E$. This allows us to create ensemble networks with the same function 
%(and accuracy) as the MotherNet but with structures that are 
%representationally richer i.e., have more parameters. Now, we 
%transition to the second phase. 
%
%\boldPara{Phase 2.}  In this phase, we co-train the MotherNet with 
%the ensemble networks. We use the whole data set to train the MotherNet 
%and use bagging to train the ensemble networks as bagging is a typical 
%and efficient method to train ensembles \cite{Dietterich2000}. During 
%this phase, we monitor the accuracy of the MotherNet and the combined 
%accuracy of the ensemble networks after every training epoch. If the 
%MotherNet results in higher accuracy, we use it to re-instantiate 
%ensemble networks through function-preserving transformations and 
%then repeat this process. If the combined accuracy of the ensemble 
%networks is higher, then we transition to the third phase.  
%%
%
%\boldPara{Phase 3.} In this phase, only the ensemble networks are trained to
%convergence. 

==> files/oracle.tex <==
%\section{Oracle Accuracy}
%
%\rev{Figure X} shows the oracle test error rate of all 
%the large ensembles trained through MotherNets i.e., the 
%test error rate if an \textit{oracle} were to pick the 
%prediction of the most accurate network in the ensemble 
%per element in the test data set. This represents information 
%the ensembles know as collections of specialists 
%\cite{Guzman2012,Guzman2014,Stefan2015}. \rev{This metric 
%is used to evaluate the effectiveness of ensembles when 
%they are applied to solve Multiple Choice Learning (MCL) 
%problems \cite{Guzman2014,Lee2016,Brodie2018}. 
%In such cases, the goal is to provide a diverse set of choices 
%that either feed into another downstream system or are presented 
%to a human being who picks from this set of diverse choices.}
%%
%\rev{We observe that the oracle test error rate keeps on improving 
%for every ensemble as we increase the number of networks. 
%This indicates that the quality of the ensemble networks 
%trained by MotherNets remains consistently good i.e., 
%well-trained ensemble networks are introduced into the 
%ensemble.} 

==> files/outline.tex <==
%\section*{Misc.}
%
%\subsection*{Typical NIPS submissions}
%
%In a typical submission, there are the following sections: 
%
%\begin{enumerate}
%	\item Introduction (1.5 pages) -- 
%	\begin{itemize}
%		\item Concise and focusing directly on what is new.
%		\item Can some time have contributions on main result toward the end. 
%		\item Sometimes, related work is deeply embedded within the introduction. 
%		\item People do use bold sub-headings. 
%		\item Motivational figures are rarely present. 
%		\item Sometimes the paper delves directly into what the problem is. 
%	\end{itemize} 
%	\item Main section (2 to 4 pages)
%	\item Experimental Section (1 to 4 pages) -- Data and benchmarks used and a
%few sub-sections, which are 
%	titled descriptively. Sometimes organized based on the data set. 
%	\item Related Work (1 or so page)
%\end{enumerate}
